Diagnosing Concept Drift with Visual Analytics

Concept drift is a phenomenon in which the distribution of a data stream changes over time in unforeseen ways, causing prediction models built on historical data to become inaccurate. While a variety of automated methods have been developed to identify when concept drift occurs, there is limited support for analysts who need to understand and correct their models when drift is detected. In this paper, we present a visual analytics method, DriftVis, to support model builders and analysts in the identification and correction of concept drift in streaming data. DriftVis combines a distribution-based drift detection method with a streaming scatterplot to support the analysis of drift caused by the distribution changes of data streams and to explore the impact of these changes on the model's accuracy. A quantitative experiment and two case studies on weather prediction and text classification have been conducted to demonstrate our proposed tool and illustrate how visual analytics can be used to support the detection, examination, and correction of concept drift.

==> Analyzing Concept Drift in Streaming Data_2/1-introduction.tex <==

\firstsection{Introduction}
\maketitle
% from the review paper of Jie Lu et al.
% To date, Artificial Intelligence and Machine Learning technologies have made immense strides in developing models and classifiers for real-world phenomena. 
To date, artificial intelligence technologies have made immense strides in developing machine learning models (e.g., classifiers) for real-world phenomena~\cite{sacha2019vis4ml}. 
% Applications of these \shixia{models} are found in fraud detection~\cite{jiang2019recent}, cybersecurity~\cite{dua2016data}, medical diagnosis~\cite{jordan2015machine}, sales predictions~\cite{dovvzan2012solving}, and countless other domains.
Applications of these models are found in fraud detection~\cite{jiang2019recent}, medical diagnosis~\cite{jordan2015machine}, sales predictions~\cite{dovvzan2012solving}, and countless other domains. 
% Often, classifiers have a built-in assumption where the mapping function of an input data used to predict an output value is static.
Often, models have a built-in assumption where the mapping function of input data used to predict an output value (e.g., prediction label) is assumed to be static.
% However, as time passes, the statistical properties of %the variable being predicted 
% \yafeng{the target domain}
However, as time passes, the mapping between the input data and the output value may change in unforeseen ways~\cite{Lu2018survey}, \liu{which could be caused by the change of the data and label.} 
In these cases, predictions made by a model trained on historical data may no longer be valid, and the model accuracy will begin to decrease over time. This phenomenon is typically referred to as \emph{concept drift} in machine learning.
% , or covariate shift, dataset shift, or non-stationarity depending on the domain. 
As more and more machine learning applications move towards streaming data, the potential for model failure due to concept drift becomes further exacerbated. \looseness=-1

% To prevent degradation of prediction accuracy, both active and passive solutions have been proposed. 

To prevent the degradation of prediction accuracy, many drift analysis methods have been proposed in the field of machine learning~\cite{iwashita2018overview, Lu2018survey}.
% , e.g.~\cite{} [ROSS: ADD SOME SAMPLE REFERENCES HERE]. 
% Another issue in the case of concept drift is that the interpretation of the historical data may also have changed over time. 
However, existing methods typically only provide a numerical drift value \mc{at each time point}. While such measures can identify when drift occurs, a single numeric cannot explain why the drift is occurring. 
Analysts need to have tools that can do more than simply alert them to when concept drift seems to be occurring. 
% Analysts and model builders need ways to understand how feature distributions have changed over time, which samples cause drift, and how they might adjust their training samples for model building. 
They need ways to understand how \liu{data} distributions have changed over time, which samples cause drift, and how the training samples can be adjusted for model building.
%Analysts need tools that can also support the identification and correction of problematic data issues. 
These underlying challenges of concept drift lend themselves well to a visual analytics paradigm in which the data and model can be \shixia{readily} evaluated for drift (``analyze first''). 
% When drift is detected, changes in data distributions and data label issues can be highlighted (``show what’s important''), and an analyst can intervene by \mc{updating the model}.
\weikairevision{When drift is detected, changes in data distribution can be highlighted (``show what’s important''), and an analyst only needs to label those drifted samples to update the model, which can save human effort.}
Once the analyst is satisfied, the system can return to the analysis state (``analyze again''). As such, we propose a visual analytics system, DriftVis, for detecting, explaining, and correcting for concept drift.

%Currently, only limited information is provided to guide the drift adaptation process. 
%When drift occurs, analysts need to relabel the impacted portion of the historical data and retrain the model. 
%However, the continuous relabeling of historical data and retraining can be an expensive, time-consuming process, which is currently not well supported.

%One major source of concept drift is the unexpected changes in the intrinsic distribution of streaming data over time~\cite{Lu2018survey}. 
%As a result, in this paper, we develop a visual analytics tool called DriftVis.
%The key idea of our approach is to tightly integrate drift analysis with interactive visualization to form an interactive and iterative drift analysis environment. 
% Our proposed tool quantifies concept drift using a distance function that measures the difference between the distributions of the historical data (used in model training) and the incoming (streaming) data. 

DriftVis has been designed to support the identification of concept drift, visually explain the drift analysis results, and enable the analysis of the root causes of such drift through a tight integration between the drift detection method and coordinated multiple views, creating a comprehensive visual analytics environment. 
\liu{As the change of data distribution is the root source of concept drift~\cite{Lu2018survey}, in this work, we focus on analyzing concept drift caused by distribution drift. Accordingly, 
the} drift detection method quantifies concept drift using a distance function that measures the difference between the distributions of the historical data used in model training and the incoming data.
In our implementation, the data distribution is modeled by an \mc{incremental} Gaussian mixture model (GMM). 
The energy distance, which is \mc{an} extension of the $L_2$ distance for measuring high-dimensional distributions, is utilized to compute the dissimilarity between two distributions~\cite{szekely2013energy}. 
This drift detection method is used to support stream- and prediction-level visualizations.
%%%% ORI
% The stream-level visualization uses a drift degree line chart and a streaming scatterplot to disclose when and where a drift might occur, and the prediction-level visualization provides an interactive analysis of the prediction model.
% \weikai{If a drift is detected, analysts can utilize the streaming scatterplot to compare the distributions over time.}
% This view combines a constrained t-SNE and a multi-step animation to explain the distribution evolution.
%%% MEGNCHEN
The stream-level visualization uses a drift degree line chart and a streaming scatterplot to disclose when and where concept drift might occur.
If drift is detected, analysts can utilize the streaming scatterplot to compare the distributions over time.
This scatterplot combines a constrained t-SNE and a multi-step animation to explain the distribution evolution.
The prediction-level visualization reveals the performance-related information of the prediction model.

%To help convey the distribution differences easily, this visualization represents the historical data as a density map and the new data as a scatterplot.
%[ROSS: I COMMENTED THIS OUT BECAUSE I THINK IT IS TOO MUCH DETAIL FOR THE INTRO, BUT IF OTHERS DISAGREE, ADD BACK IN]\yafeng{To help convey the distribution differences easily, this visualization has two modes.
%The scatterplot mode represents the historical data as a density map and the new data as a scatterplot.
%The density diff mode presents the relative density change between the current data batch and its previous batch.

In order to demonstrate the capabilities of our system, we have conducted two case studies exploring the drift in weather prediction and academic paper topic evolution.
%We demonstrate how DriftVis can identify possible causes of drift and support analysts in adapting their model \yafeng{to the} drift as necessary. 
A demo prototype of the system is available at \url{http://conceptdrift.thuvis.org/}.
The main contributions of our work include:
\begin{compactitem}
% \item\noindent{\textbf{A visual analytics tool} for detection, investigation, and correction of concept drift in streaming data.
\item\noindent{\liu{\textbf{A visual analytics system} for detection, examination, and correction of concept drift.}}
% \item\noindent{\textbf{A distribution-based drift detection method} to quantify the drift degree of a data stream over time.}
\item\noindent{\liu{\textbf{A distribution-based drift detection method} to quantify the drift degree over time.}}
\item\noindent{\textbf{A streaming scatterplot} to explore the distribution changes over time and identify the root cause of concept drift.}
\end{compactitem}

% It leads to a phenomenon that the predictive behavior of the model changes over time in unforeseen ways.
% Concept drift research involves the development of methodologies and techniques for drift detection, understanding and adaptation.
% This becomes a critical and challenging issue in the era of big data where the data distribution often changes over time.


% The difference between concept drift and overfitting should be emphasized.

==> Analyzing Concept Drift in Streaming Data_2/2-related.tex <==
% !TEX root = EvoTree-KDD.tex

\section{Related Work}
\label{sec:related-work}
% \subsection{Concept Drift Detection}
%All the papers can be found in the related work folder in google drive
%https://drive.google.com/drive/u/0/folders/13dBB5yBeXRWzxKiN5oPPGqgMBxVa9PEJ

%some of them may appear more than once in the following lists
%
%%followings are some surveys
%


% Our work focuses on detecting, explaining and correcting concept drift. In this section, we review recent work on concept drift analysis and visual performance analysis as it relates to model building.

% \subsection{Concept Drift Detection}
\subsection{Concept Drift Analysis}
% As previously stated, concept drift is a phenomenon in which the distribution of a data stream changes over time in unforeseen ways, causing prediction models built on historical data to become inaccurate. 
Research related to concept drift can be categorized into two main topics: drift detection and drift adaptation~\cite{Lu2018survey}.

\noindent \textbf{Drift Detection.} 
% The detection of concept drift has been a key research area. 
Error-rate-based methods and data-distribution-based methods are the most popular drift detection methods. 
% The error-rate-based approaches~\cite{baena2006early, gama2004learning} estimate the error rate of a model on the new test data by labeling a part of the test data.
% A drift is then defined as the time point when a significant statistical increase or decrease in the error rate occurs.
The error-rate-based methods~\cite{baena2006early, gama2004learning} monitor the online error rate of a model based on ground-truth labels.
A drift is detected if there is a significant increase in the error rate.
% Gama et al.~\cite{} proposed a pioneering framework, Drift Detection Method, which monitors the error-rate and gives a confidence interval on it.
% Several works improved the framework under different aspects.
% For example, Baena-Garc{\i}a et al.~\cite{} used the distances between two classifications instead of counting the number of errors to improve the detection of gradual concept drift.
% Fr{\'\i}as-Blanco et al.~\cite{frias2014online} improved the calculation of the confidence interval with Hoeffding inequality.
% Liu et al.~\cite{liu2017fuzzy} changed the conventional time window to a fuzzy time window so that two time windows can overlap, which can handle the gradual concept drift better and yield better performance on drift detection.
These methods are less efficient in practice as it is often challenging to acquire high-quality data labels for calculating the error rate of streaming data.

Distribution-based techniques do not rely on data labels.
Instead, these techniques directly detect concept drift by calculating the distribution change \ross{with respect to} the \mc{streaming} data, which is a major cause of concept drift.
A key challenge for distribution-based techniques is how to measure the distribution change by calculating the distance between two data distributions.
Kifer et al.~\cite{kifer2004detecting} used total variation, which is one of the earliest attempts to use a distance function for drift detection.
Webb et al.~\cite{webb2016characterizing, webb2018analyzing} measured the distribution difference using the Hellinger distance and total variation.
\mc{In their work,} the drift degree was measured in different attribute subspaces, such as joint distribution and class distribution.
%He [ROSS: IS He THE NAME OF A PERSON, OR IS THIS FROM WEBB ET AL? IF DIFFERENT WORK, MISSING CITATION, IF SAMe WORK, CAN'T SAY HE] measured the drift degree in different attribute subspaces, such as joint distribution and class distribution.
% $P(Y)$, conditioned marginal covariate distribution $P(X\mid Y)$ and posterior distribution $P(Y\mid X)$.
% A simple drift visualization was also developed, which combines a line chart showing the degree of drift over time and a grid visualizing the degree of drift of each pair of data attributes.
% However, it discretizes all numeric attributes into five bins and then measures the difference between distribution, which harmed its accuracy.

%In our tool, we utilize a distribution-based method as these methods need no ground-truth labels. Furthermore the distribution-based methods can identify which parts [ROSS: WHAT DO WE MEAN BY PART? FEATURE?] of the data causes concept drift, which is useful in facilitating the understanding of concept drift.
In our system, we utilize a distribution-based concept drift detection method, as these methods do not need ground-truth labels.
Furthermore, distribution-based methods can identify the samples in the streaming data that cause concept drift, which is useful for facilitating the understanding of concept drift.
Specifically, we model the streaming data distribution by an \mc{incremental} GMM and apply the energy distance \ross{function}~\cite{rizzo2016energy} to measure the distance between distributions.\looseness=-1
%Specifically, we model the streaming data distribution by an \mc{incremental} GMM and apply the energy distance \ross{function}~\cite{rizzo2016energy} to measure the distance between data distributions.
% The energy distance calculation does not have any underlying assumptions on the data distribution nor any discretization.

% Methodologies and techniques in concept drift research have been developed to detect when and where the drift occurs and adapt learned knowledge to the model.
% As related to our contributions, we briefly introduce the typical works in drift detection and drift adaption. 
% Drift detection has been studied the most and popular methods include 
% Error rate-based drift detection techniques track the error rate and 

% The system will alarm the drift if the error rate increase and exceed the confidence interval.

%xxx can also help explain how the drift occurs and where the distribution changes the most in the data. It has been shown that xxx has a state-of-the-art performance. 
%As such, we use xxx as our drift detection algorithm. 

%We use distribution-based drift detection and model ensemble for drift adaptation. 

%The difference between our work and anomaly detection should be emphasized.

\noindent \textbf{Drift Adaptation.} 
% If drift is detected, models must be adapted to account for differences between the streaming data and the original training data. 
Drift adaptation focuses on improving the model performance on \mc{the streaming data} by updating the existing learning model to \ross{account for} the drift. %new test data
Existing methods of drift adaptation include model retraining and ensemble methods~\cite{Lu2018survey}.
% most of the works also provide the solution to handle the concept drift.
% Drift adaptation is the strategy we use to update the existing learning model according to the drift.

Model retraining retrains a new model with a combination of the new data and old data to replace the old model. 
The main problem encountered with these types of methods is doc{determining} how much of the \mc{old} data will be discarded and how much of the new data will be utilized in training~\cite{bach2008paired}.
%Ensemble methods use a set of base learners and partially adjust these base learners to adapt to the drift.
\yafeng{Ensemble methods comprise a set of base learners and} \mc{adjust the base learners} when adapting to the drift.
\mc{Typical adjustments include} adding new base learners, updating \mc{existing} base learners, removing unsatisfactory base learners, and \mc{changing} the weights of base learners in the ensemble model.
%Compared with model retraining, ensemble methods are more efficient because they do not require a full retraining of the model.
%Furthermore, ensemble methods are capable of handling reoccurring drift by reusing old base learners.
%Thus, we mainly focus on introducing the ensemble-based adaption methods.
% Some works focus on extending the classical ensemble model to handle the concept drift, including bagging~\cite{oza2001experimental,bifet2010leveraging}, boosting~\cite{chu2004fast} and random forest~\cite{li2015learning,gomes2017adaptive}.
Hulten et al. proposed a tree-based method, CVFDT~\cite{hulten2001mining}, which replaced the sub-tree exhibiting poor performance with a retrained sub-tree.
The dynamically weighted majority method~\cite{kolter2007dynamic} down-weights the classifier that makes a wrong decision and up-weights the classifier that makes a correct decision.
When the ensemble \mc{model} makes a wrong decision, it will train a new base learner and add it to the ensemble, and the base learners with low weights will be removed.
%Learn$^{++}.$Net~\cite{elwell2011incremental} re-weights the base learners based on the performance on the last batch [ROSS: LAST BATCH OF WHAT? DATA?] to prevent adding new base learners too frequently.
Learn$^{++}.$Net~\cite{elwell2011incremental} re-weights the base learners based on the prediction performance on the latest streaming data to prevent adding new base learners too frequently.

\yafeng{Compared with model retraining, ensemble methods are more efficient because they do not require a full retraining of the model.
Furthermore, ensemble methods are capable of handling reoccurring drift by reusing old base learners.}
In DriftVis, we employ the method proposed by Kolter et al.~\cite{kolter2007dynamic} due to its competitive performance and flexibility.
% DriftVis supports several adjustments for ensemble methods, such as constructing new base learners by selecting data of interest and re-weighting old base learners by measuring the similarity between the new data and the training data of base learners.
% So we do not require the groundtruth labels to compute the accuracy and adjust the weights.

% we choose the ensemble model because of its flexibility, and reweight the base learners according to the similarity between the training data and streaming data.


% The locally adjusting strategy can be used when model supports the local adjustment.

% 
% Other works adaptively change the weights of base learners according to the incoming data.

% For example, Paired Learners~\cite{bach2008paired} maintained two learners, the stable one and the reactive one, simultaneously.
% The stable leaner uses all data since last replacement, while the reactive one uses only $w$ most recent data.
% When the performance of the reactive learner surpasses the stable one, it will replace the stable leaner with the reactive one.
% ADWIN~\cite{bifet2007learning} increases the window size as the new data comes.
% When it finds that the current window can be divided into two parts with a significant difference, the old part will be discarded, and the new part will be preserved and used in training a new model.




\subsection{Visual Performance Analysis}
% Existing efforts in visually analyzing streaming data can be classified into three categories: understanding of streaming data, improvement of model performance.
% While the machine learning community has developed a variety of methods for analyzing model performance, the visual analytics community has also focused on creating tools to support the performance analysis of machine learning models. 
% Existing efforts on visual performance analysis of machine learning models can be classified into two categories: understanding model performance, and; debugging and improving models~\cite{choo2018visual,liu2017towards}. 
Existing efforts in visual performance analysis of machine learning models can be classified into two categories~\cite{choo2018visual,liu2017towards}: 1) understanding the model performance; 2) debugging and improving models. 

\noindent\textbf{Understanding model performance}. 
There are a variety of visualization tools that have been developed to support analysts in exploring the performance of machine learning models. 
Tzeng et al.~\cite{Tzeng2005} developed a visualization tool to support the performance analysis of artificial neural networks utilizing a graph-based visualization.
%The main objective of this tool is to aid in the selection of the model parameters, such as the model structure. 
%Another tool, 
ModelTracker~\cite{amershi2015modeltracker} was developed to convey both the overall and instance-level performance of a binary classifier. 
Squares~\cite{ren2017squares} extended the work from ModelTracker and was designed to illustrate and compare the prediction score distributions of multiclass classifiers.
% Ming et al. extracted a set of rules to approximate the complex model and then developed a visual interface to explain the decision logic of the model~\cite{ming2019rulematrix}.
More recently, there has been a major focus on supporting the understanding of the performance of deep neural networks~\cite{choo2018visual,Hohman2019Visual,yuan2021survey}, such as convolutional neural networks~\cite{bilal2018convolutional,hohman2020summit,jia2019visualizing,rauber2017visualizing,wongsuphasawat2018visualizing}, recurrent neural networks~\cite{ming2017understanding,strobelt2018lstmvis}, deep Q-networks~\cite{wang2019dqnviz}, and deep generative models~\cite{kahng2019gan}.
While the majority of work has focused on supporting specific models, there has also been work focusing on developing model-agnostic interactive visualization tools to support model understanding~\cite{ming2019rulematrix,wexler2020if,zhang2019manifold}.
In general, the goal of many current systems is to support analysts in understanding the performance characteristics of models from multiple perspectives and illustrate which model features contribute to the performance.

\noindent\textbf{Debugging and improving models}.
Along with tools for understanding models, a variety of tools have been developed to support debugging and improving machine learning models.
These efforts focus on exploring the reasons why a learning process does not work as expected and supporting analysts in refining the model.
Liu et al.~\cite{liu2017towards} proposed a directed-acyclic-graph-based visualization method to illustrate how data flows through a network in the training process and thus facilitates the diagnosis of a failed training process.
%It supports the debugging of observed failure of a learning process by enabling the analysis of neurons at multiple facets. 
DeepEyes~\cite{pezzotti2018deepeyes} was developed to help analysts identify the potential issues that deep neural networks may experience in the training process, such as redundant filters and inadequately captured information. 
Other research has explored model diagnosis of a variety of deep neural networks, such as deep generative models~\cite{liu2018analyzing,wang2018ganviz}, recurrent neural networks~\cite{kwon2019retainvis}, and deep sequence models~\cite{ming2020protosteer,strobelt2019seq}.
% Researchers have also some initial efforts to analyze the robustness of deep neural networks and diagnose the root cause of the robustness issues~\cite{cao2020analyzing,liu2018robustness,ma2020explaining}.

One current drawback with model debugging and performance improvement is the lack of generalizability. Models (or classes of models) often have specific parameters and features that are not completely generalizable.
%The aforementioned work focus more on understanding the model performance and improving the performance by modifying the model structure and/or parameters. 
As a result, most existing methods of visual model performance analysis are model-dependent. 
However, concept drift is a generalizable problem that focuses on understanding how data has shifted over time. Our system is designed around understanding shifts in streaming data and exploring distributions, making our proposed system model-independent.
%aims to analyze concept drift in streaming data predictions.
%The developed method is based on the distribution of data. 
%Thus, it is model-independent. 
%Moreover, a streaming scatterplot is developed to disclose the distribution difference between different data batches over time.
This is similar to current work that focuses on analyzing the robustness of learning models in terms of data quality, such as understanding model vulnerabilities to adversarial examples~\cite{cao2020analyzing,liu2018robustness,ma2020explaining} and detecting out-of-distribution samples~\cite{Chen2020}.
These methods also compare training data with test data, identify outliers, and then analyze their effects on the model performance.
While inspired by the same motivation of enhancing the training dataset, our work differs from these methods in two ways. 
First, instead of considering only one static test dataset, we handle a stream of test data, where new test data keeps on coming in and then is appended to the existing data. 
Second, we measure the concept drift using a distribution-based method, which models the streaming data distribution by an incremental GMM. 
To illustrate the drift over time and the root cause of such drifts, a streaming scatterplot is developed, which combines the advantages of the constrained t-SNE and a density map. 

%%Lujie 2018 Learning under Concept Drift: A Review
%Webb 2016 Characterizing Concept Drift
%GAMA 2013 A Survey on Concept Drift Adaptation
%Zliobait 2010 Learning under Concept Drift an Overview
%Tsymbal 2004 The problem of concept drift definitions and related work
%followings are published in 2018/2019
%Lujie 2019 Fuzzy Clustering-based Adaptive Regression for Drifting Data Streams
%% https://ieeexplore.ieee.org/abstract/document/8688575
%Lujie 2018 Learning under Concept Drift: A Review
%% https://ieeexplore.ieee.org/abstract/document/8496795
%Lujie 2018 Accumulating regional density dissimilarity for concept drift detection in data streams
%% https://www.sciencedirect.com/science/article/abs/pii/S0031320317304636
%Lujie 2018 Active Fuzzy Weighting Ensemble for Dealing with Concept Drift
%% https://www.atlantis-press.com/journals/ijcis/25888775
%followings are published in and before 2017:
%Lujie 2017 Fast concept drift detection using singular vector decomposition
%% https://ieeexplore.ieee.org/abstract/document/8258835
%Lujie 2017 Concept drift region identification via competence-based discrepancy distribution estimation
%% https://ieeexplore.ieee.org/abstract/document/8258734
%Lujie 2017 Fuzzy competence model drift detection for data-driven decision support systems
%% https://www.sciencedirect.com/science/article/abs/pii/S0950705117303751
%Lujie 2017 Fuzzy time windowing for gradual concept drift adaptation
%% https://ieeexplore.ieee.org/abstract/document/8015596
%Lujie 2017 A fuzzy kernel c-means clustering model for handling concept drift in regression
%% https://ieeexplore.ieee.org/abstract/document/8015515
%Lujie 2017 Regional concept drift detection and density synchronized drift adaptation
%% https://opus.lib.uts.edu.au/handle/10453/126374
%Lujie 2016 An Online Competence-Based Concept Drift Detection Algorithm
%% https://link.springer.com/chapter/10.1007/978-3-319-50127-7_36
%Lujie 2016 Fuzzy user-interest drift detection based recommender systems
%% https://ieeexplore.ieee.org/abstract/document/7737835
%Lujie 2016 A concept drift-tolerant case-base editing technique
%% https://www.sciencedirect.com/science/article/abs/pii/S0004370215001459
%Lujie 2014 Concept drift detection based on anomaly analysis
%% https://link.springer.com/chapter/10.1007/978-3-319-12637-1_33
%Lujie 2014 Concept drift detection via competence models
%% https://www.sciencedirect.com/science/article/pii/S0004370214000034
%the follows are distribution-based method
%Alippi 2016 A pdf-Free Change Detection Test Based on Density Difference Estimation
%Alippi 2017 An Incremental Change Detection Test Based on Density Difference Estimation
%Lujie 2017 Regional Concept Drift Detection and Density Synchronized Drift Adaptation
%Lujie 2016 A concept drift-tolerant case-base editing technique
%Lujie 2016 Concept Drift Detection Based on Equal Density Estimation
%the follows are error-based method
%Lujie 2017 Fuzzy Time Windowing for Gradual Concept Drift Adaptation

==> Analyzing Concept Drift in Streaming Data_2/3-system.tex <==
\begin{figure*}[!tb]
\centering
{\includegraphics[width=\linewidth]{fig/system-overview.pdf}}\hfill
\vspace{-3mm}
%\caption{DriftVis overview. The drift detection module takes the streaming data and training data as input and generates the drift value and GMM result. The drift visualization module illustrates the drift with both line chart and scatterplot to facilitate the understanding of the drift. User can update the model through the visualization and trigger the drift adaptation method.}
\caption{DriftVis overview.
When data streams in, an incremental Gaussian mixture model is first employed to model the data, and the output is further used in drift detection and data visualization.
The stream-level visualization displays the drift degree and the time the distribution changes to support drift analysis.
%, so that users can understand when, where and why drift happens.
The prediction-level visualization facilitates the understanding of the model performance for drift adaptation.
\yafeng{The training data in the adapted prediction model will be used for drift detection in the next iteration.}
%The adjusted training data will be used for drift detection if users update the model and adapt to the drift.
}
\vspace{-5mm}
\label{fig:system-overview}
\end{figure*}


\section{Requirement Analysis}


% http://visgroup.thss.tsinghua.edu.cn:49620/

% http://conceptdrift.thuvis.org/

This work is driven by previous research on concept drift and our discussions with a researcher from the China Meteorological Administration (E$_1$) and three machine learning practitioners (E$_2$, E$_3$, and E$_4$) regarding their needs for model deployment in real-world applications.
%E$_1$ focuses on training machine learning models to predict the probability of rain for the China Meteorological Administration.
E$_1$ works on weather predictions.
E$_2$ focuses on predicting whether a computer motherboard meets the quality standards for a computer manufacturing company, Inventec.
E$_3$ and E$_4$ are machine learning researchers and are interested in classifying conference papers to facilitate their research,
% We have been collaborating with E$_1$ and E$_2$ in other projects and 
and E$_4$ is a co-author of this paper.
% Regular meetings are conducted throughout our collaboration. 
A central problem each of these experts faces after deploying a machine learning model is how to monitor the model performance over time and decide when the model needs to be updated if an unsatisfactory performance is identified.
%[ROSS: HOW WERE DISCUSSIONS DONE? HOW MANY DISCUSSIONS? NEED SOME MORE DETAILS HERE.]

% \subsection{Requirement Analysis}
To understand the experts' needs, we engaged in weekly free-form discussions with our \yafeng{experts} for two months to learn about the systems they were currently using for model performance analysis, and what challenges they faced when using these systems.
In our discussions, the \yafeng{experts} commented that there are already several cloud-based model performance monitoring services.
Two widely-known services are Google's continuous evaluation service~\cite{Google_continue} and the data drift detection service on Microsoft Azure~\cite{MS_drift}.
These services can alert analysts when drift occurs.
However, they do not support the exploration of where the data distribution has changed.
This requires the analyst to spend more time investigating
\yafeng{which subset of the most recent data could benefit the prediction model the most}
and then labeling the data before retraining the model. 
Our experts noted that if the system could help identify where the distribution changes occurred, the amount of labeling could be reduced. %providing savings in time as well as costs for labeling.
% Neither of them are satisfactory to them.
%Google's service continuously needs human labelers to provide groundtruth labels for streaming data, which can make the monitoring cost prohibitively high. 
% The cost of Google's continuous evaluation service is too high for them because it needs human labels to evaluate the performance of the model on new data. 
% \shixia{As a result, it} is desirable to provide a tool that directly relies on the data itself to save cost.
%At this point, 
%However, the data drift detection service on Microsoft Azure provides more support for labeling.
%The Microsoft service directly compares training data with the stream of test data and generates a line chart to show the drift degree as well as the contribution of each feature to the drift over time.
\mc{This is favored by the experts because the cost of acquiring a large number of data labels is usually high.}
% Furthermore, the experts noted that having a tool that requires data labeling only when necessary, e.g., when concept drift is detected, it would be beneficial as their workflow often cannot justify the cost of adding more labels to a dataset. 

%This service can help discover whether and when concept drift happens, but is less capable of helping users explore the underlying cause of the drift.

% The unsatisfactory part of the service is that it lacks effective visualizations to explain the drift analysis result and help users
% It utilizes \shixia{line charts} to .
% However, with the \shixia{aforementioned} information, the question of ``where the drift happens'' cannot be answered.
% \shixia{The line charts can well illustrate when the drift happens. 
% However, they cannot ''}
% Such discussions above 

% Based on the discussions and the observed limitations of current drift detection tools, we focused on developing a visual analytics tool for detecting the occurrence of concept drift and, more importantly, supporting the \mc{analysis of the root cause of the drift} and correction of the drift.
% To insure the usefulness of our tool, we engaged in a user-centered design process. We held biweekly discussions with our practitioners, iterated on designs, and summarized the requirements for the visual analytics tool.\looseness=-1
Based on the literature review, the observed limitations of current drift detection methods, and the discussions with experts, we summarized the requirements for the visual analytics system as follows:

% DriftVis is designed following the guideline of "analyze first," "show the important," and "analyze further"~\cite{keim2008visual} by integrating drift detection, drift visualization, and results after adaption.


% From MS: In the context of machine learning, data drift is the change in model input data that leads to model performance degradation. It is one of the top reasons where model accuracy degrades over time, thus monitoring data drift helps detect model performance issues.
% To monitor for data drift, a baseline dataset - usually the training dataset for a model - is specified. A second dataset - usually model input data gathered from a deployment - is tested against the baseline dataset. Both datasets are profiled and input to the data drift monitoring service. A machine learning model is trained to detect differences between the two datasets. The model's performance is converted to the drift coefficient, which measures the magnitude of drift between the two datasets. 

%\noindent \textbf{R1. Detecting potential concept drift in the stream of test data.}
% \noindent \textbf{R1. Detecting when concept drift happens in streaming data.}
\noindent \liu{\textbf{R1. Detecting when concept drift happens}.}
Concept drift is one of the major causes of model accuracy degradation over time.
To tackle this issue, many methods have been proposed to track and detect when drift occurs in streaming data~\cite{gama2014survey,Lu2018survey,street2001streaming}.
%\mc{For example, E$_2$ once found that his quality control algorithm failed because a new batch of base board with different board height is used in the assembly line.}
All the experts expressed that they required a convenient way to alert them to the potential occurrences of concept drift during the running process of their deployed machine learning models. 
For example, E$_2$ once found that his quality control algorithm wrongly judged some qualified motherboards to be unqualified because a new batch of motherboards used in the assembly line did not have the same board height as before.
Thus, it is critical to detect potential concept drifts in \mc{streaming data} and inform the analyst to minimize the decrease in accuracy and quickly recover from the drift process.
% On the other hand, the experts also pointed that updating prediction models to adapt to the drift often requires human effort to label additional training data.
% The cost of data labeling is not trivial and on top of the requirement of detecting concept drift, they would also like to reduce false alarms as much as possible.
% [ROSS: DO WE DO ANYTHING WITH FALSE ALARMS?]
% \mc{The experts also noted that without using labels, drift detection could not be 100$\%$ accurate, i.e., introducing false alarms to the users.
% To this end, we cannot solely rely on the calculated drift degree and need an interactive tool to verify whether the detected data drift will actually influence the model performance.}
% The experts also noted that the drift detection could not be 100$\%$ accurate.
% To this end, we cannot solely rely on the calculated drift degree and need an interactive tool to verify whether the detected data drift will actually influence the model performance.
%Concept drift detection does not only attracts a lot of research attentions~\cite{Lu2018survey} but also gradually employed in machine learning model deployment on cloud~\cite{Google_continue, MS_drift.

%However, a major issue is the cost of continuously updating labels. E$_2$ commented that ``The major concern is the cost. Using a machine learning model instead of a human quality inspector is targeted at reducing cost. If the human quality inspector is continuously needed, then the benefit of the machine learning model is questionable.''
%As such, the practitioners desire a method without the need of getting the ground-truth labels of the test data.
%The experts also agreed that without using the labels, the drift detection could not be 100$\%$ accurate.
%\yafeng{The experts also noted that without using labels, drift detection could not be 100$\%$ accurate.}
%To this end, an interactive tool is needed to verify whether the detected data drift will actually influence the model performance.
%Such a goal cannot be achieved by using the calculated concept drift degree alone.
%[ROSS: THE LAST COUPLE SENTENCES HERE DON"T MATCH THE OVERALL REQUIREMENT AND MAY BELONG TO A DIFFERENT REQUIREMENT.]
% That is also a reason that they decide to collaborate with us to develop a visual analytics system, instead of . 
% The problem of GR
% Although only from the data itself, the drift detection is not 



% Detecting the drift serves as the basis in handling the concept drift. 
% In the data drift detection service on Azure, it is a central component 

%\noindent \textbf{R2. Analyzing the detected drift.}
\noindent \textbf{R2. Analyzing where and why drift happens.}
%As stated above, we need extra human efforts to analyze the detected drift.
% As previously stated, we need to analyze the detected drift before we can effectively address the data issue.
%A basic such analysis is verifying whether the detected data drift will actually influence the model performance.
All the experts expressed a strong need for analyzing where and why drift occurs after it is detected and understanding how the detected drift will influence the model performance. 
% A critical task is understanding how the detected drift will influence the model performance.
Thus, a simple numerical measure of drift degree is not sufficient.
%E$_1$ commented that ``The change of features can help in this task as we know which features are important. If there are significant changes on these features, it is highly possible that the performance will change.''
For example, experts usually want to know how each feature has changed over time.
E$_3$ commented, ``We know which features are important to the model, and if there are significant changes in these features, the drift is likely to affect the model performance.''
Other useful information to explore \mc{includes} the distribution of the data and their changes over time.
% Here, the experts wanted to explore if the density of some regions in the data changed or if new regions of data are emerging. 
The experts wanted to quickly locate the regions dominated by new data or the regions where the data distributions have changed. 
In these cases, the model performance is likely to have a drop.
%Besides the verification of the detected drift, the analysis of the root cause of the drift is also helpful.
In addition to exploring where drift happens (e.g., which feature and where it is in the data distribution), the analysis of why \mc{the drift} happens is also important. %it
E$_4$ said, ``Knowing why the drift occurs really helps to take necessary actions - sometimes the action \yafeng{may} not even be required on the model side. 
For example, several months ago, I found that the model performance degradation was simply caused by the changed position of the camera. 
It was moved to another angle, resulting in the incoming video not being the same as the training dataset.''
% \mc{These requirements (analysis of where and why) are well aligned with previous research on concept drift mining~\cite{Lu2018survey}.}
The need to analyze where and why is \yafeng{also} well aligned with previous research on concept drift analysis~\cite{liu2017regional,Lu2018survey, wang2020conceptexplorer}.


\noindent \textbf{R3. Overcoming drift and improving performance.}
Having an understanding of the drift is not the end of the analysis.
Experts needed to appropriately adapt the model to the new data and improve the performance, which is called drift adaptation.
%The simplest adaptation approach is labeling a subset of the streaming data, which causes the drift, and fully retraining a new model \mc{incorporating} the labeled data.
\yafeng{The most straightforward adaptation approach is to retrain the model with additional labeled streaming data.}
However, the \yafeng{experts} were not in favor of this method.
E$_3$ commented, ``For us, a lighter-weight method is more practical. It is inefficient to retrain the whole model as it often takes hundreds of GPU hours.''
E$_2$ also desired to shorten the time of drift adaptation because 
the quality control of the computer motherboard assembly line is crucial and would have a large influence on the brand.
\yafeng{Fast reactions to any detected issues on the computer motherboard assembly line can reduce company losses.}
% More importantly, due to privacy issues, we are often not allowed to train a model with the incoming data.''
% and new-data-free adaption approaches.
E$_1$ further pointed out that there were sometimes reoccurring patterns in the weather data, such as revolving seasons and day-night alternations.
% Thus, part of knowledge in the old model is still valuable.
Thus, it is desirable to have a drift adaptation method to reuse part of the old model.
This is also reflected in the current research trend that ``adaptive models and ensemble techniques have played an increasingly important role in recent concept drift adaptation developments~\cite{Lu2018survey}.''\looseness=-1


% Requirements:
% 1. detect drift in streaming data
% 2. understand the root cause of the occurring drifts
% 3. overcome the drift and improve performance. 





==> Analyzing Concept Drift in Streaming Data_2/4-driftvis.tex <==


\section{Design of DriftVis}
\label{sec:DriftVisDesign}
%\subsection{System Overview}
\label{sec:system}


%Motivated by the discussions and requirements, 
DriftVis is designed to detect, analyze, and overcome concept drift.
It consists of three modules: drift detection, drift visualization, and drift adaptation (Fig.~\ref{fig:system-overview}).

%introduce each module
% [ROSS: IS THIS THE RIGHT WAY TO PHRASE THIS? IS IT STREAM OF TEST DATA OR JUST INCOMING/STREAMING DATA?]
The \textbf{drift detection} module compares the training dataset with the \yafeng{latest} streaming data and calculates the drift degree over time (\textbf{R1}).
% \yafeng{[YAFENG: is this correct to say 'batch' and 'test data stream'?]}
An incremental GMM is employed to model the data distribution, and a distribution-based drift detection method is developed to calculate the drift degree.
% [ROSS: WAS THIS DEVELOPED OR APPLIED? IS THE GMM NEW?][Weikai: The main idead from IGMM, which update the component with the data one by one. We improve it a little in our scenario.] 
% The details of this module are introduced in Sec.~\ref{sec:DriftDetectionMethod}.
Detecting drift in streaming data serves as the basis for the subsequent analysis, including discovering the root cause of the detected drift and adapting the model to compensate for it.\looseness = -1

The \textbf{drift visualization} module provides an exploratory analysis of when, where, and why drift happens (\textbf{R1}, \textbf{R2}).
Such analysis is primarily supported by a streaming scatterplot that shows the data distribution over time.
Combined with the drift degree line chart and a feature selection list, analysts can make informed decisions on how to adapt the model to overcome the drift.
% Details of the drift visualization module are introduced in Sec.~\ref{sec:visualization}.\looseness=-1

% to compare the distributions over time
% displays the drift value over time and projects the original data into the scatterplot.
% Users can examine , and then choose to add a base learner to handle the novel data if necessary.

The \textbf{drift adaptation} module adapts the learning model to \mc{the unforeseen change in streaming} data (\textbf{R3}).
%There are two categories of available drift adaptation methods~\cite{Lu2018survey}: model retraining and ensemble methods.
%Ensemble methods do not require fully retraining the model and thus are more efficient. %than model retraining. 
%Furthermore, if reoccurring drift happens, ensemble methods provide the flexibility to reuse \mc{existing base} learners by adjusting the weights of these learners.
%Thus, 
In \minorchange{DriftVis}, we employ the ensemble method developed by Kolter et al.~\cite{kolter2007dynamic} due to its competitive performance and flexibility.
In particular, we train a set of base learners on different subsets of the historical data.
%In particular, we train many [ROSS: HOW MANY IS MANY?] base learners on different subsets of the historical data.
\mc{These base learners are combined with different weights to adapt to the new data} and improve performance. 
% Such an ensemble model has two advantages.
% First, an ensemble model can be improved simply by adding a base learner, as opposed to completely discarding the previous model and retraining a new one, which is costly.
% Second, if reoccurring drift happens, the ensemble model provides the flexibility to reuse the previous learners by adjusting the weights of the base learners.

Our \yafeng{contributions} mainly focus on the first two modules, so we introduce them in detail as follows. 

\subsection{Drift Detection}
\label{sec:DriftDetectionMethod}
% Detecting concept drift in streaming data (\textbf{R1}) serves as the basis for the subsequent analysis, such as discovering the root cause of the detected drift (\textbf{R2}) and adapting the model to compensate for drift (\textbf{R3}).

% The developed density-based concept drift detection method includes two steps: a direct drift degree calculation based on the given data samples and a fine-tune calculation to avoid drift over-estimation. 

% \noindent \textbf{Drift degree calculation}.
% Concept drift is defined as the unforeseen changes of mapping between the input data and the output value.
One major source of concept drift is the unexpected changes in the intrinsic distribution of the data stream~\cite{iwashita2018overview, Lu2018survey}.
Thus, a key challenge to compute the drift degree is how to measure the difference between data distributions. 
\textbf{Energy distance} is motivated by the potential energy between objects in a gravitational space~\cite{rizzo2016energy}.
The distance is zero if and only if the two distributions are identical.
% The major advantages of energy distance are: 1) distribution free; 2) its calculation is linear to the number of dimensions and can be easily scaled to high dimensions~\cite{goldenberg2018survey}. 
The major advantage of energy distance is that its calculation is linear to the number of dimensions and can be easily scaled to high dimensions~\cite{goldenberg2018survey}. 
As a result, we employ energy distance to measure the drift degree.
% To calculate the change in the data distribution, we use the energy distance~\cite{szekely2013energy}, which is a generalization of the widely-used L2-norm distance.
% The energy distance is also used in industrial concept drift detection services~\cite{MS_drift}.
For two groups of data samples $X = \{{x}_1,\ldots,{x}_n\}$ and $Y = \{{y}_1,\ldots,{y}_m\}$, the energy distance of their underlying distributions is defined as:
\begin{equation}
\label{eq:drift_origin}
% d(X,Y)=\dfrac{2A-B-C}{2A},
d(X,Y)=(2A-B-C)/2A,
\end{equation}
where $A=\frac{1}{mn}\sum_{i=1}^{n}\sum_{j=1}^{m}\lVert {x}_i-{y}_j\rVert$ is the average of the pairwise distance between two groups of samples, $B=\frac{1}{n^2}\sum_{i=1}^{n}\sum_{j=1}^{n}\lVert {x}_i-{x}_j\rVert$ and $C=\frac{1}{m^2}\sum_{i=1}^{m}\sum_{j=1}^{m}\lVert {y}_i-{y}_j\rVert$ are the averages of pairwise distance within $X$ and $Y$, respectively.
Here $\lVert{x}\rVert$ is the L2-norm of vector ${x}$\looseness=-1.
% The calculated distance represents how likely a concept drift occurs between two timestamps, i.e., the larger the distance, the more likely a concept drift exists.
%In DriftVis, the drift degree at time $t$ is calculated from training set $X_0$ and the incoming data $X_t$ at time $t$ in the data stream.
%In practice, data samples may come one at a time, such as the daily weather prediction.
%In that case, we use the incoming data in a sliding window \weikai{that ends} at time $t$. to get a more accurate estimation of the drift degree.
% \yafeng{In DriftVis, the drift degree at time $t$ is calculated by the energy distance between the training set $X_0$ and the incoming data $X_t$ in a sliding window that ends at time $t$ in the data stream.}
% 
%This is different from the typical settings in concept drift detection papers where drift degree is commonly calculated between two adjacent time points $t$-$1$ and $t$.

In DriftVis, the drift degree at time $t$ is \yafeng{measured} by the energy distance between the training set $\hat X$ and the streaming data $X_t$ at time $t$.
\mc{In practice, data samples may come one at a time, such as daily weather data.
In that case, $X_t$ is set as the streaming data in a sliding window ending at time $t$ to reduce noise and get a more accurate drift degree.}
% \yafeng{Different than the typical settings in concept drift detection where drift degree is calculated on adjacent time points, we always compare the latest streaming data to the training set.}
% We made this choice because, in practice, the \yafeng{experts} are more interested in how streaming data is different from the training data.
% Such differences are the root causes of the potential drops in model performance.
%The drift of adjacent batches of test data more focus on describing the temporal changes in the stream of test data.
%It is also valuable but not the focus of DriftVis.
%\yafeng{The drift of adjacent time points describes the temporal changes in the stream and tends to overestimate drift as it does not account for the historical data.
%By testing adjacent batches, alerts for reoccurring drift are captured; however, this type of drift may not need to be addressed if the model has learned from the previous occurrence.}
% Another reason is that calculating the drift between adjacent time points will always alert the reoccurring drift (e.g., the seasonal change of the weather records), which may not need to be addressed if the model has learned it from the previous occurrence.
% During the development of DriftVis, we find that 
In the development of DriftVis, we found that directly calculating the drift degree between $\hat X$ and $X_t$ may overestimate the drift.
This typically occurs when $\hat X$ contains several clusters, while $X_t$ only contains a subset of these clusters.
% This often happens in practice because the size of the training data is usually larger than that of the incoming data. 
For example, $\hat X$ may contain the weather \yafeng{records} for a whole year, \yafeng{but} $X_t$ only contains one month of data.
In this example, the calculated distance is large because $X_t$ lacks the samples from other months.
However, the model performance drop is not large since the distribution of $\hat X$ already covers that of $X_t$. 
As a consequence, directly calculating the distribution distance can potentially generate false alarms.

To tackle the issue of drift over-estimation, it is desirable to compare $X_t$ with only the training samples that are similar to them. 
The key challenge is, for each newly arrived data sample, how to select the similar training samples, and how many samples are enough. 
A straightforward solution is to use the $k$-NN algorithm to select the top-$k$ similar training samples.
Although this method is able to reduce the drift over-estimation to some extent, experts \yafeng{have to tune}
%' efforts are needed in tuning 
the parameter $k$ for different datasets and even for different samples to achieve good results, which is impractical in applications.
To solve this problem, we let the data speak for itself, i.e., automatically determining the similar samples based on the data sample clusters in the dataset.
\mc{Compared with $k$-NN, the number of clusters of a clustering algorithm can often be automatically determined with unsupervised model selection methods, such as Akaike information criterion (AIC)~\cite{akaike1998information} and Bayesian Information Criterion (BIC)~\cite{schwarz1978estimating}.}
The intuition behind this solution is that in the same cluster of the dataset, the samples are similar.
Thus, at each time $t$, we first incrementally cluster the data samples $X_t$ at time $t$ based on the clustering result before $t$.
Then, based on the new clustering result, for each sample $x_t^i$ in $X_t$, we select the training samples that are in the same cluster of $x_t^i$ as its similar samples.
% i.e., selecting all the samples in the cluster

% we model the fine-grained structure in the streaming data and training data, i.e., finding the internal clusters in the data. 
% find the belongings of the data samples in the test data to the clusters of training data. 
% common clusters in the training data $X_0$ and the $t$-th batch of test data $X_t$.
\mc{Due to streaming nature of the data, we employ an incremental clustering method in DriftVis, i.e., the incremental GMM algorithm~\cite{engel2010incremental}}.
% The incremental clustering method we employ in DriftVis is .
A GMM-based clustering method is utilized because GMM is able to approximate almost any continuous distribution where the value of each feature is continuous~\cite{bishop2006pattern}.
% Given $X_t$, the algorithm incrementally update the clusters instead of intuitively re-calculating a new GMM using the expectation–maximization (EM) algorithm~\cite{bishop2006pattern}.
% % Due to the streaming nature of the data, we employ an incremental GMM, which incrementally clusters the data samples into set of Gaussian components as data stream in.
% Compared with the intuitive re-calculation method, the employed incremental GMM has two advantages.
% First, re-calculation of a GMM is time-consuming and prohibits real-time interaction for streaming data.
% Second, re-calculation at each time point may introduce unstable clustering results because the EM algorithm finds a local minimum for a GMM~\cite{bishop2006pattern}.
% As a consequence, for adjacent time points, the EM algorithm may converge to different local minimum and introduce instability in the drift visualization, which utilizes the clustering results. 
% The incremental GMM is able to cluster the data $\hat X \cup \{X_t \mid 1 \leq t\}$ into a set of Gaussian components (clusters).
% models the training data $X_0$ and the streaming data $\{X_t \mid 1 \leq t\}$ as a mixture of Gaussian components (clusters).
% We adopt GMM in DriftVis because 
% and incrementally assigns data samples in the test data to existing clusters or creates new clusters if necessary.
% points models and data as an evolving mixture of to 
% find the common clusters in the training data and the stream of test data.
% A Gaussian mixture model assumes that the data contains several clusters, and each cluster can be modeled by a Gaussian distribution.
% We adopt GMM in DriftVis because it is able to approximate any continuous distribution.
% to [ROSS: TO AN ARBITRARY ACCURACY or WITH AN ... ?] arbitrary accuracy. 
% The developed incremental GMM is able to further align the clusters in the two batches, e.g., $X_0$ and $X_t$.
% the detected clusters in the adjacent batches.
% \weikai{An example of clustering result is shown in Fig.~\ref{fig:teaser}, where nine components are used to model the data distribution.}
The incremental GMM algorithm can be split into an offline clustering step for the training dataset $\hat X$ and an online clustering step that ingests data samples $X_t$ for each time point $t$:

\begin{figure*}[!tb]
\centering
{\includegraphics[width=\linewidth]{fig/fig3.pdf}}\hfill
\vspace{-3mm}
\caption{DriftVis analysis workflow. When drift is detected, analysts can explore when, 
where, and why it happens with the help of stream-level visualization.
To adapt to the drift, analysts can select data samples to build learner(s) and then update the model.}
\label{fig:workflow}
\vspace{-4mm}
\end{figure*}

\noindent \textbf{Offline Clustering.}
A GMM is built to cluster the data samples in $\hat X$, where each cluster is a Gaussian component $N(\cdot \mid \mu, \Sigma)$ with mean $\mu$ and covariance $\Sigma$.
% $p(x^i) = \sum_{k=1}^{K} \pi^k N(x^i|\mu^k, \Sigma^k)$.
% Here $x^i$ is the $i$-th data sample in the training data $\hat X$.
% $N(x|\mu,\Sigma)$ denotes a Gaussian distribution with mean $\mu$ and co-variance $\Sigma$.
% $\pi^k$ is the weight of each Gaussian distribution.
% To determine the number of clusters, we use the Bayesian Information Criterion (BIC)~\cite{schwarz1978estimating} to select the best model that simultaneously has a high likelihood and low model complexity.
The number of clusters is determined by the Bayesian Information Criterion (BIC)~\cite{schwarz1978estimating}.
% We use an EM algorithm to get a maximum likelihood estimation of the GMM parameters: $\mu^k$, $\Sigma^k$, and $\pi^k$.


\noindent \textbf{Online Clustering.} 
The major purpose of this step is to incrementally cluster the data samples in $X_t$. 
% updating $\mu^k$, $\Sigma^k$, and $\pi^k$ given the data samples at time $t$.
%To detect concept drift caused by data samples that are different from all previous data samples, we \yafeng{should} also allow for the creation of new clusters if necessary.
%To this end, 
For each data sample $x_t^i$ in $X_t$, we need to decide %whether it belongs to an \yafeng{existing} cluster or if a new cluster should be created.
\yafeng{which existing cluster it belongs to or if a new cluster should be created when it is not close to any existing cluster.}
If the probability of this sample belonging to an existing Gaussian component $p=N(x_t^i|\mu, \Sigma)$ is higher than a threshold (0.95 in DriftVis), we assign the data sample to the cluster with the maximum probability and update the mean and the covariance of the corresponding Gaussian component~\cite{engel2010incremental}.
% If the probability is larger than a threshold (), the data sample is considered to belong to an old Gaussian component.
% To incorporate the historical information, we update the 
% \mc{The the mean and co-variance of the old component is also updated} 
Otherwise, there should \weikai{exist}{be} a new Gaussian component \weikai{which}{that} better fits the current data sample.
% The intuition is that we assign the instances to the previous components if possible and build new components for the remaining instances.
% For each data instance in the new data, we calculate the likelihood of the instance \yafeng{belonging to each component.}
% If this maximum of the likelihood is still smaller than a threshold, the instance is regarded as a novel instance and will be stored in a temporary set.
% The threshold is set to the $1\%$ quantile of the likelihood of existing instances.
Constructing a Gaussian component from a small number of samples cannot accurately estimate the component's mean and covariance, and will bring instability to the clustering result.
To solve this problem, we temporarily assign these samples to the Gaussian components with the maximum probability.
\weikairevision{When enough such samples are identified, we build a new GMM using these samples and then merge the new components into the current clustering results. In DriftVis, to get enough samples and to avoid creating noisy components, we set the threshold to be half of the average component size or we allow the analyst to set a specific threshold value.}
%\weikairevision{When enough such samples (we choose half of the average component size or a given threshold here to prevent creating noisy components) are identified, we build a new GMM using these samples and then merge the new components into the current clustering results.}
% It is straightforward to merge two mixture models since each model can be regarded as a set of Gaussian components.
Based on the clustering result at $t$, we calculate the drift degree $D_t$ between $X_t$ and $\hat X$ as a weighted sum of the drift degree for each cluster:\looseness=-1
% weighted sum of the drift degree between each pair of the matched clusters: 
\begin{equation}
\label{eq:drift_weighted}
D_t = \sum_i \frac{|X_t^i|}{|X_t|}d(X_t^i, \hat X^i),
% + \frac{|X_t^{-1}|}{|X_t|} 
\end{equation} 
where $|\cdot|$ is the number of samples in a set and $d(\cdot)$ is the energy distance.
$\hat X^i$ and $X_t^i$ are the samples of the $i$-th cluster in $\hat X$ and $X_t$, respectively.
% which belong to the $i$-th cluster, and $X_t^i$ are the samples in $X_t$ belonging to the $i$-th cluster.
%For \yafeng{any new cluster,}
For a cluster that satisfies $|\hat X^i|=0$, we set the drift $d(X_t^i, \hat X^i)=1$ because the data samples in $X_t^i$ are unlike other samples in the training dataset and will probably cause model performance drop.
In this case, there should be a larger drift degree.
% \mc{This also reflects }
% in the training data and is the set of data samples that are assigned to $X_0^i$.
% $X_t^{-1}$ is the set of data samples that do not belong to any existing clusters and trigger the incremental GMM to create new clusters.
% The intuition behind Eq.~\ref{eq:drift_weighted} is that the overall drift degree we treat the drift drgree between the drift degree
%Next, we introduce the basic idea of incremental GMM, i,e, how to cluster the training data and the streaming data.
% how to assign data samples to existing clusters and determine whether a new cluster is needed.
% = \{ x | x \in X_t \wedge x \in X_0^i \}$ the and $X_t^i$ are the $i$-th matched clusters in the training data $X_0$ and test batch $X_t$, and $|.|$ denotes the number of the data samples in that cluster.
%ROSS: I DON'T THNK YOU NEED THIS SENTENCE, BUT IF YOU FEEL OTHERWISE ADD IT BACK IN. In the next subsection, we introduce our incremental Gaussian Mixture Model.
% To handle new clusters in the test batch, the drift $d(X_t^i,X_0_i)$ will be set to $1$.
%The Gaussian mixture model 
%As shown in Fig.~\ref{}, for each data batch, the mixture model approximates the real data distribution by a set of weighted Gaussian distributions.
% So we can assigns each data sample to the most likely Gaussian distribution, and hence have a more accurate estimation of the drift degree.
% In particular, for two sets of data $X$ and $Y$, we first partition $X$ and $Y$ according to the Gaussian Mixture Model as $X = \{X_1,...,X_m\}$ and $Y = \{Y_1,...,Y_m\}$, where $X_i$ is the i-th Gaussian distribution.
% Based on this partition, we calculate the drift degree as 
% \subsection{Incremental Gaussian Mixture Model}
% \label{subsec:IGMM}
% As stated above, the basic idea of the incremental GMM is finding the belongings of data samples in the test data to the clusters in the training data. 
% Correspondingly, the algorithm can be split into two steps: (1) an offline step to cluster the data samples in the training data, and (2) an online step that checks whether a data sample in the test data belongs to existing clusters or a new cluster appears.

% \noindent \textbf{Data distribution modeling}. 
% As part of the drift degree calculation, 
% The modeling of data distribution is very important for the developed drift detection method.
% As the GMM can approximate almost any data distribution~\cite{bishop2006pattern}, we utilize it to model the data distribution.
% In particular, the incremental GMM developed by Song et al.~\cite{engel2010incremental} is employed to model the streaming data. 
% Intuitively, for each time point $t$, one could directly construct a GMM for all available data: $\{X_s \mid 0\leq s \leq t\}$ and apply the widely-used expectation–maximization (EM) algorithm~\cite{bishop2006pattern} to solve the model.
% However, there are two drawbacks of this straightforward GMM application.
% To tackle these problems, we propose an incremental GMM that incrementally updates the model for the incoming data at time $t$.
% By incrementally updating the model, instead of re-building a GMM for each time point, we achieve better stability and are able to support \mc{real-time interaction} in DriftVis.
% \weikai{[FOR EACH TIME POINT or FOR ALL TIME POINTS?]}

% in the temporary set using the same method and then merge the new mixture model with the previous one.
% hold such samples in an individual set and . 

% After examining all the instances in the new data, we check whether the size of the temporary set is large enough to build new components.
% If so, we build a new GMM on the instances in the temporary set using the same method and then merge the new mixture model with the previous one.

% If the size of the temporary set is insufficient, we will assign those novel instances to the components with the highest likelihood directly, but the temporary set will be kept and enlarged when more data stream in.


% The incremental Gaussian mixture model () is used to find the common data modes in the training data $X_0$ and the batches in the test data $X_1, ..., X_t, ...$, where $X_t$ is the $t$-th batch.
% The model approximates the data distribution of each $X_i$ by a linear combination of Gaussian distribution:



% We use GMM [ROSS: BUT WE USE IGMM, RIGHT? NOT GMM? SO SHOULD THIS BE WE INITIALLY USED A GMM?][\weikai{I think this sentence is duplicated with a previous one.}] to model the incoming data because it is capable of approximating any continuous distribution~\cite{bishop1995neural}.
%Thus, our approach is not restricted to data that satisfies particular distribution.
% \yafeng{Thus, our approach does not require a priori knowledge of the data distribution.}

% One approach to modeling the distributions is to independently construct a GMM for each data batch.
% However, this approach ignores the inline relationship between the historical data and the new data.
% To avoid this issue, we developed an incremental Gaussian Mixture Model.
% This model generates [ROSS: THIS SENTENCE WASN"T FINISHED?]




% Since we do not know how many components should be included in the mixture model to model the distribution well, 
% When new data is ingested, instead of training a new GMM on all available data, we first use the previous result to accelerate the process of building a GMM.




% [One thing is that the components with too few points will be removed in the implementation. The points in such components will be assigned to the remaining component with highest generative probability, and also go into the temporary set. I am not sure how to write all this clearly..]

% \subsection{Energy-distance-based Drift Calculation}

% As these changes may happen in hidden variables which cannot be \mc{computed explicitly}~\cite{liu2017regional}, the concept drift is often detected via the temporal change of the target streaming dataset distribution~\cite{Lu2018survey}:
% \begin{equation}
% \label{eq:1}
% P_{[0, t]}(X) \neq P_{[t+1, \infty]}(X),
% \end{equation}
% where $X$ is the target streaming dataset, $P_{t_1}(X)$ and $P_{t_2}(X)$ are the distributions $P$ of the dataset $X$ at time $t_1$ and $t_2$.
% If Eq.~\ref{} is satisfied, there is a concept drift at time $t$.
% % , and $d (.,.)$ is a distance function measuring the difference (change) between two \mc{timestamps}.
% As the groundtruth dataset distribution at a timestamp is unknown, we need to statistically test whether the data distribution of two timestamps are equal from 

% we use an \mc{unbiased} estimator to estimate the value of the energy distance.

% \mc{In DriftVis, we adopt the energy distance~\cite{} to calculate the distance $d$ between the distributions of two timestamps for the following reason.}


% To estimate the value more accurately, the estimator takes in the data samples from a time range instead of a single timestamp and calculates the value as:

% improves upon a distribution-based drift detection model
% compares the distribution between the historical data and new data.
% Unlike the traditional drift detection which compares the distribution between two consecutive time windows (the old one and the new one), our drift detection used the training data as the historical data, because we are more interested in those unforeseeable data.
% Even though the distribution of data changes over time, we will not regard it as the drift if the new distribution has been covered by our model.

% trash
% Thus, to faithfully detect a concept drift, we need a metric to measure the difference between the subset of the target streaming dataset of \mc{two timestamps}.
% As enumerating all the statistical properties of a dataset is computationally infeasible, we use the distribution of the target datasets to represent the
% Mathematically, suppose we have a streaming dataset $X = \{ x_i \}$, where each $x_i$ is a tuple of the actual data $d_i$ and a timestamp $t_i$. 

% \subsection{Drift Detection}

% We should carefully discuss the metric/distance that we used to measure the drift.
% Since the distribution of data varies greatly, we prefer to use a distribution-free method, to measure the difference between distributions directly (i.e., we do not have any assumption that the data follow a particular distribution).
% Otherwise, we need to estimate the distribution first, which is usually computationally problematic and even infeasible to deal with high-dimensional data.
% Therefore, many widely used distance, such as Hellinger distance, Total variation distance, and KL-divergence, cannot be used here.
% Finally, we choose \textbf{energy distance} here, which can be thought of as a generalization of $L_2$ distance between two distribution.
% One advantage is that the energy distance will be zero if and only if two distributions are identical, and hence we can use it to detect the concept drift.
% Another advantage is that it is distribution-free and can scales well to high dimensions, so that it can handle the data in different scenarios.

% A significant advantage of the energy distance is that $d(X, Y) = 0$ if and only if X and Y are identically distributed.
% Thus, the energy distance has been used for testing of equal distributions
% Another advantage of energy distance is that it is distribution free, i.e., the estimated value of energy distance does not depend on the distribution form of random vectors.
% from "Multivariate global sensitivity analysis for dynamic models based on energy distance"
% KL-divergence is also widely used in computer science. 
% The maximum of KL is infite... The maximums of JS is log2 in fact.
%Since the distribution of data varies greatly, we prefer to use nonparametric 
%Kernal density estimation is a classical nonparametric method is model the distrbution.
%Gaussian mixture model could have better capability to deal with high-dimensional data.
% Once the distribution is obtained, there are lots of statistical distance that have been proposed to measure the distance between two distribution.
% Total variantion distance...
% KL-divergence is also widely used in computer science.
% Wasserstein distance...


%As shown in Fig.~\ref{}, there are two kinds of data samples: data samples for training the model and the incoming test data samples.
%Correspondingly, there are two kinds of data drifts: (1) the drift between training data and testing data, and (2) the drift between testing data at different timestamps.
%Both two concept drifts reflect


%We can now calculate the drift of the streaming data by calculating the energy distance between two consecutive time windows.
%More specifically, the drift value on time $t$ is set as the energy distance between the data in window $[t-w,t)$ and $[t,t+w)$, where $w$ is the size of the window.
%We name it ``\textbf{origin drift}'' since it indicates the inherent drift in the data itself.
%However, despite the fact that the distribution before drift is different from the distribution after drift, the performance of the learning model may not be affected if both of them are well covered by the training data.
%In this case, the drift can be handled by the learning model and thus not so critical.
%Therefore, \textbf{our drift} aims to compare the distribution between training data and new data.
%The drift value will be low if the new data are covered by the training data well.
%Here we borrow the idea of a drift adaptation algorithm, LDD-DSDA~\cite{liu2017regional}, which resamples a new batch of training data from the historical data to adapt the new data.
%When calculating \textbf{origin drift}, we will not use the entire training data for calculating the energy distance.
%Instead, for each point in the new data, we search its nearest neighbors in the training data and then form a batch.
%The energy distance will be calculated between this batch and the new data.



\subsection{Drift Visualization}
\label{sec:visualization}

%Visual sedimentation https://www.aviz.fr/Research/VisualSedimentation. https://ieeexplore.ieee.org/document/6634152/

%Working with the underlying distribution-based drift detection method and ensemble drift adaption method, the visualization of DriftVis has two major components: the stream-level visualization to analyze the drift in the stream data and the prediction-level visualization to assist the adaption of the prediction model.

%\subsubsection{Overview}
% Provide an overview of the visualization components here and introduce the analysis workflow.
To support the analysis of \mc{when, where, and why drift happens (\textbf{R1}, \textbf{R2}),} DriftVis employs two visualization components, a stream-level visualization (Fig.~\ref{fig:teaser}(a)) and a prediction-level visualization (Fig.~\ref{fig:teaser}(b)).
%These two components work together to support an iterative and progressive drift analysis process.
%\noindent\textbf{Stream-level visualization}.
% \yafeng{The stream-level visualization discloses the distribution changes of the data stream over time. It is application-independent and supports the exploration purely on the data, including the distribution of data samples, the drift detection results, and some of the raw data contents (e.g., the raw text before feature extraction), without any information regarding the prediction model. }
The stream-level visualization discloses the distribution changes of the data stream over time. It %is application-independent and 
supports the exploration purely of the data, including the distribution of data samples, the drift detection results, and some of the raw data contents (e.g., the raw text before feature extraction).
%Leveraging our drift detection method, the goal of this visual component is to illustrate when and where drift might have happened and support the exploration of the cause of the drift. 
%A line chart (Fig.~\ref{fig:teaser}B) is used to show the detected drift degree over time and the resulting drift degree after model adaptation. 
%Seeing a ramping on the line chart indicates that a drift is likely to happen, and this step can serve as a starting point for concept drift analysis. 
%Along with the line chart, a streaming scatterplot (Fig.~\ref{fig:teaser}D) is designed to visually explain the distribution changes. 
%This view uses the GMM components 
%\weikai{built in Sec.\ref{sec:DriftDetectionMethod}} 
%to group data samples and compares the distribution between the recent streaming data and historical data.
%The streaming scatterplot supports the discovery of any new Gaussian components or data distribution shifts in the existing components. 
%Emerging components reveal that a subpopulation of the recent streaming samples follows a distribution not covered by the historical data.
%The shift of existing components indicates that the current model does not well explain the new data even though the new data is following a distribution that is similar to the historic data.
%The streaming scatterplot view has two modes, scatterplot and density diff, which are described in section~\ref{subsec:streamLevelVis}.
%\noindent\textbf{Prediction-level visualization}.
\yafeng{The prediction-level visualization focuses on the performance-related information of the prediction model and reveals how the adaptation to the drift affects the model performance (\textbf{R3}).}
%Integrating with the ensemble-based drift adaptation method, the goal of this component is to enable ensemble model updates by taking the insight from drift analysis and disclosing the changes in the prediction results. 
%This component shows a list of base learners available to build the ensemble model, a list of data batches in the order of occurrence, and a performance view displaying the prediction accuracy on selected data samples.
%\noindent\textbf{Analysis workflow}.
The drift detection and adaptation methods support the two visualization components and serve as the foundation for the concept drift analytics environment.\looseness=-1 

%Fig.~\ref{fig:workflow} illustrates the typical analytics workflow of using DriftVis to identify and explore the drift, and adapt the prediction model to the drift.


Fig.~\ref{fig:workflow} illustrates the typical analysis workflow as data streams in. 
The workflow begins with an analyst checking the drift degree line chart \yafeng{to detect any obvious drift increase (``when'')}.
\yafeng{In cooperation with the ``when'' analysis, the analyst can further analyze ``where'' and ``why'' the drift happens on the streaming scatterplot, which illustrates}
if the \yafeng{incoming data} forms new components, \mc{deviates from the existing components or causes density increase/decrease in some regions.}
% noticeably deviates from the existing components. 
%\mc{Using the scatterplot,} it is easy to identify the occurrence of new components and \mc{deviations from the existing components.}
%\yafeng{However, it is non-trivial to identify local density changes when the overall region doesn't transform.}
%However, it is non-trivial to \mc{visually compare the region density in two time oints}. %measure the shift when the new data %%deviates from the existing components
%To better illustrate such \mc{density change}, the user can switch between the two different modes of the streaming scatterplot and use the density diff mode to investigate the increase and decrease of the density by comparing the new data to the historical data.
After \yafeng{confirming a drift}, the analyst can select data samples on the scatterplot to build new base learners. % on the selected data. 
Using the available base learners, the analyst updates the ensemble and 
%Once the analyst is satisfied with the data distribution coverage and the new drift degree, the analyst can 
checks if the model performance has improved using the \yafeng{prediction-level} views. 
This workflow can be applied iteratively as new data streams in.\looseness=-1

\subsubsection{Stream-Level Visualization}\label{subsec:streamLevelVis}
The stream-level visualization is designed to illustrate and explain concept drift \yafeng{- specifically, the calculated drift degree and the density change}. It consists of a drift degree line chart (Fig.~\ref{fig:teaser}A), a feature selection list (Fig.~\ref{fig:teaser}B), and a streaming scatterplot (Fig.~\ref{fig:teaser}C).
%On the data importer a user can load the dataset and use the `Add Data' button to bring in the next batch of streaming data. 
%This provides a way DriftVis simulates the ongoing of the streaming data. 
The drift degree line chart is used to alert the analyst of possible occurrences of concept drift by displaying the calculated drift degree over time (\textbf{R1}). 
The line chart coordinates with the feature selection list to turn on and off the drift degree lines calculated on different features.
When any single feature is selected, the y-axis can switch between the drift degree and the feature value.
\weikairevision{We used the line chart because it is the most common form of time series visualization~\cite{Heer2009, liu2017towards}.\looseness=-1}
% The drift degree is calculated from our drift detection algorithm and is updated upon any model adaptation. 
% The feature value is smoothed using a moving average.
%For streaming data, we visualize historical data with a compact time axis but expand the most recent data to a wider space. 

%Only warning that a drift might have occurred is insufficient for overcoming the drift.
As described in requirement \textbf{R2}, it is critical to know where \yafeng{and why} drift occurs by exploring the change of data distribution over time.
%We employ a streaming scatterplot with two different visualization modes to support the detection and analysis of the drift.% through answering the question of where by deeply diagnosing data distribution change. 
%First, we visualize the data distribution and then compare the distribution between the new data and the historical data. 
We use a GMM-based constrained t-SNE to \mc{continuously} project the streaming data onto a 2D space and have designed two visualization modes, scatterplot and density diff, to present the data for distribution-based analysis. 

% \mc{The basic requirements for the scatterplot are (1) the readability at each time point and (2) the stability between two time points.}
% These two requirements are well grounded by previous research~\cite{liu2014topicpanorama, Xiang_VAST2019}.
% In addition, as we want to find the drift caused by deviating data samples from their components, we need to preserve the overall structure in each component.
% To this end, we develop a GMM-based constrained t-SNE.
% 
\noindent\textbf{GMM-based constrained t-SNE.} 
The GMM-based constrained t-SNE is designed to 1) preserve the \yafeng{sample} similarities in the original high dimensional space, 2) explain the distribution of each Gaussian component, and 3) minimize the movements of previous data points in the t-SNE plot when new data \yafeng{streams in}. 
%While t-SNE~\cite{maaten2008visualizing} preserves similar data points close to each other in high probability, 
% Our GMM-based constrained t-SNE leverages the output of the \mc{incremental GMM} in the drift detection method and adds three constraints to t-SNE~\cite{maaten2008visualizing} to better project the distribution of each component with respect to the position of the historical data points. 
The state-of-the-art solution to achieve the aforementioned goals is the supervised t-SNE developed by Choo et al.~\cite{choo2013utopian}, where \yafeng{samples} in the same class are grouped together by reducing their distances \yafeng{using} a shrink factor.
Although shrinking the projection within each group can reduce the visual clutter between groups and \yafeng{improve} readability, \yafeng{it} does not consider the dispersion of each group and 
\yafeng{could also not maintain stability when the projection updates with additional data.}
%is unstable when new data is added.
% To overcome these limitations, we modified the shrink factor with respect to the dispersion of each GMM component \yafeng{in our first constraint} and added \yafeng{two more constraints}.
To overcome these limitations and well convey the distribution patterns of Gaussian components, we modify the shrink factor with respect to the dispersion of each component \yafeng{and add two constraints to improve the stability of the shape of Gaussian components and data positions.}
%add a stability factor, and preserve the overall shape of each component. 
\looseness =-1

\mc{As we assume that the ground-truth labels are unavailable when calculating the projection,} the shrink factor uses the component label inferred from the incremental GMM. %instead of supervising the projection using class labels. 
%\mc{The shrinking factor is used to reduce the within-component distance of data samples and enlarge the between-component distance.}
% We add a shrink parameter to the within component distances to data points within a component closer together and separate the different \mc{Gaussian components}.
Its value \yafeng{is weighted by} the component dispersion that highly dispersed components will shrink more.
In DriftVis, we use entropy to measure dispersion.
For each Gaussian component $C_k$ whose covariance matrix is $\Sigma_k$, the shrink factor $\alpha_k$ is determined \yafeng{as follows:}
%by \mc{the dispersion of each Gaussion component (In DriftVis, we use its entropy $H$)}, \mc{the maximum allowed shrinking} factor $\alpha$ and a \mc{weighting} factor $\beta$: %global shrink component shrink
\begin{equation}
    \alpha_k = \alpha\cdot\left(1- \beta\cdot \frac{H[C_k]}{\max_{k'}\{H[C_{k'}]\}}\right).
\end{equation}
Here \mc{$\alpha$ is the maximum allowed shrinking} factor, $\beta$ is a \mc{weighting} factor, and $H[C_k]$ is the entropy of the Gaussian distribution of component $C_k$.
In practice, \mc{to ensure that the calculated shrink factor does not exceed the maximum, $\alpha$}, we enforce $H[C_k]$ to be no smaller than a small positive $\epsilon$. Thus, $H[C_k] =\max( \frac{1}{2}\ln{|\Sigma_k|} + \frac{D}{2}(1 + \ln{2\pi}), \epsilon)$, and $D$ is the size of the feature dimension. 
For the most dispersed component, $\alpha_k = \alpha\cdot(1-\beta)$, and 
\yafeng{for the least dispersed component $\alpha_k \approx \alpha$.}
Adding this factor to the distance calculation yields, 
\begin{equation}\label{eq:dist}
\text{dist}({x}_i, {x}_j) =\left \{
\begin{array}{ll}
\alpha_k\cdot\|{x}_i- {x}_j\| & {x}_i, {x}_j \in C_k \\
\|{x}_i- {x}_j\| & \text{otherwise}
\end{array}.
\right.
\end{equation}


To further improve the stability of the projection results, we add two constraints into the supervised t-SNE:

The first is a shape constraint that maintains the shape of each Gaussian component to be stable between adjacent time points.
% To this end, we add a constraint on relative distance of each data sample to the center of its belonging Gaussian component.
Suppose we have $n$ \yafeng{samples} of original data and $m$ new \yafeng{samples} from the streaming data.
The $n$ original \yafeng{samples} form $k$ original Gaussian components.
As the shape is hard to measure, we approximately maintain the relative distances between the original $n$ data samples and the component centers. 
% \mc{The relative distances of $m$ new data samples are not maintained because we do not have that information in the current time point.}
This is achieved by minimizing the KL-divergence between $P_c$ and $Q_c$ $\in \mathbb{R}^{n\times k}$, which represent the joint probability distributions of the similarities between the $n$ original samples and the $k$ center constraint points in the high dimension and low dimension, respectively.
Each center constraint point is taken as the gravity center of the Gaussian distribution in the high dimensional space and its corresponding low dimensional projection in the previous iteration.
Following t-SNE, the distributions $P_c$ and $Q_c$ are defined as:
\begin{equation}
    \begin{array}{rl}
       (P_c)_{ik} &= w_k\cdot\exp(-\text{dist}({x}_i, {x}_k)/2\sigma^2)\\
       (Q_c)_{ik} &= (1+ \|{y}_i- {y}_k\|^2)^{-1} 
    \end{array}.
\end{equation}
Here, $w_k$ is the weight for the $k^{th}$ center constraint and is set to $\sqrt{\lvert C_k\rvert}$, where $\lvert C_k\rvert$ is the sample number in the $k^{th}$ Gaussian component. ${x}_i$ is the high dimensional vector of the original instance, and ${x}_k$ is the high dimensional center of the Gaussian component $C_k$,
and ${y}_i$ and ${y}_k$ are their projected low dimensional coordinates. $\text{dist}({x}_i, {x}_k)$ uses Eq.~(\ref{eq:dist}).

The second constraint is to maintain the positions of the original samples.
%To improve running efficiency, we use blue noise sampling~\cite{balzer2009capacity} to select $n^\prime$ samples from $n$ original samples and introduce a virtual constraint point for each. 
\lu{To improve the run-time efficiency, when sample size $n$ is greater than 500, we use blue noise sampling~\cite{balzer2009capacity} to select $n^\prime$ (500) samples from $n$ original samples and introduce a virtual constraint point for each.}
$P_s$, $Q_s$ $\in \mathbb{R}^{n\times n^\prime}$ represent the joint probability distributions of the similarities between the $n$ original samples and the $n^\prime$ selected samples.
When sample $x_i$ is used as the $k^{th}$ virtual constraint point, $(P_s)_{ik} = 1$, and this will restrict the change of the projected coordinates of the $n^\prime$ selected samples and maintain the position stability of the overall projection.
% R3Q4
%\weikairevision{We use $n^\prime=\min\{n,n_{\max}\}$ to restrict the maximum of the number of constraints. We set $n_{\max}=500$. in our implementation}.\looseness=-1

Combining the above two constraints and the supervised t-SNE, we obtain the projection by minimizing the objective function:
\begin{equation}\label{eq:cost}
    \lambda\cdot KL(P\|Q) + \varphi\cdot KL(P_c\|Q_c) + (1 - \lambda - \varphi)\cdot KL(P_s\|Q_s).
\end{equation}
Here $KL(\cdot\|\cdot)$ is the KL-divergence between two distributions.
The first term \mc{is the original optimization goal of supervised t-SNE that minimizes the difference between the high-dimensional distribution $P$ and the 2-D distribution $Q$ of all the $m+n$ \yafeng{samples}.
The second and third terms are the shape and the position constraints, respectively.}

% \yafeng{Large component is considered as stable structure and we want to ensure a higher resilience of their shape. %using a higher similarity between the component center and the samples in this component. 
% Thus, the pairwise similarities are calculated as follows:}

% }
% To further improve the readability of the Gaussian components and the stability of iterative drift analysis, \yafeng{we add a constraint on component centers to preserve the overall structure and a constraint on \mc{a subset of} original samples to retain their projected positions.}
% \mc{At each time point,} we have $n$ \yafeng{samples} of original data and $m$ new \yafeng{samples} from the streaming data

%and for each of the components we introduce one constraint point for the component's center.
%We use blue noise sampling to select $n^\prime$ samples from the $n$ original instances and add one virtual constraint point for each selected sample. %[ROSS: WHAT IS "THEM" HERE? - Yafeng: sampled instance].
% To compute the projected coordinates, we \mc{add the above two constraints regarding component centers and samples to the original  \yafeng{objective function} in t-SNE:}
% minimize a combination of three Kullback-Leibler(KL)-divergences.

%takes all $n+m$ samples and applies the original t-SNE minimization \yafeng{using the distance function in Eq.~\ref{eq:dist}}. 

% The second KL-divergence is trying to keep position stability by adding constrains on original samples. To improve running efficiency, we use blue noise sampling~\cite{} to select $n^\prime$ samples and introduce a virtual constraint point for each.
% $P_s$, $Q_s$ $\in \mathbb{R}^{n\times n^\prime}$ represent the joint probability distributions of the similarities between the $n$ original samples and the $n^\prime$ selected samples.
% When sample $x_i$ is used as the $k^{th}$ virtual constraint point, $(P_s)_{ik} = 1$, and this will restrict the change of the projected coordinates of the $n^\prime$ selected samples and keep the position stability of the overall projection.

% The third KL-divergence is added to keep shape stability of Gaussian components for better distribution analysis. 
% To achieve this goal, for every original Gaussian component, we introduce one constraint point for the component center and preserve the distances between the center and the samples in the same component.
 %and takes the component dispersion into effect [ROSS: SINCE WE REFER TO THE EQUATION, DO WE NEED TO SAY "TAKES THE COMPONENT DISPERSION INTO EFFECT"?]. 



\noindent\textbf{Scatterplot and density diff.}
To visually explain the distribution and the drift, the streaming scatterplot utilizes two modes, scatterplot and density diff.
\emph{Scatterplot mode} uses a density representation to display the historical data distribution and scattered points to represent streaming data. 
All data samples are projected using the GMM-based constraint t-SNE projection but rendered differently.
% All data samples are projected using the GMM-based constraint t-SNE projection.
% Historical data is rendered using density areas where we use light haze to represent deeper and lighter densities. 
Historical data is rendered using a density map where a lighter color represents a lower density. 
On top of the density map, the streaming data is displayed as scattered points. 
Categorical colors are used to separate the Gaussian components.
%The streaming data subpopulation assignments in the GMM is also encoded by color. 
Fig.~\ref{fig:teaser}C shows an example of the scatterplot mode %where the scattered points are 
for analyzing
\mc{the papers from NeurIPS.}%an academic conference.}
% the daily weather records in the current stream.
% In this figure, we can observe that the yellow points are likely to follow a different distribution as they could not be described by the blue Gaussian component. 
%This mode supports the comparison between all historical data and the streaming data or between the historical data a selected base learner is trained on and the streaming data. 

To illustrate the change of data distribution, we utilize a two-stage animation
to \yafeng{exhibit} the appearance of incoming data samples.
%, which runs when new data is added.
The first stage updates the projection of historical data and the density map.
Historical data points move from their original positions to their updated ones as the new streaming data is used in the projection calculation.
As this movement occurs, a new density map will be constructed using the updated projection of the historical data points.
The second stage draws the new streaming data where data points are grouped based on their Gaussian component assignment and displayed by group.
%The first stage shows the movement of historical data points from their original project, to their updated positions as the density area is reconstructed with the additional streaming data. [YAFENG - IS THIS CORRECT?]
%From where they were projected, these points move to their new positions and reconstruct density areas. [ROSS: DON'T UNDERSTAND, IS THIS STILL REFERING TO THE HISTORICAL DATA? NEEDS CLARIFICATION]
%As this updates, the older density areas and the scattered points will disappear and join the new areas. 
%The second stage is to plot data points from the stream. 
%These data points are grouped based on their Gaussian component assignment and displayed by group. 
%The data point appears near the center of its group and moves to its projection target position given by the GMM-based constrained t-SNE.

The \emph{density diff mode} is used to illustrate \mc{the density change} of data distribution by visualizing the density difference between two \yafeng{datasets, which can be} consecutive data batches 
\yafeng{or two batches selected by the analyst.}
%or between the data used in a selected base learner and the current batch. 
%\yafeng{[AFTER WE TAKE STREAMING DATA, WHICH DATASETS ARE BEING COMPARED HERE?]}
% Even though t-SNE does not preserve density, it can reflect the relative density change between iterations with addition of the virtual constraint points.
To gauge the density difference, this view uses grids to represent the 2D space and calculates the percentage of data points falling into each grid in the \yafeng{latest streaming data.}
%most recent batch from the stream. 
For the grid on the $i^{th}$ row and $j^{th}$ column with $n$ data points, its \yafeng{normalized} \mc{density} is
% [ROSS: add "is" here, does that make sense?] 
$grid^t_{i,j} = n /N$ where $N$ is the number of data points at time $t$.
To produce a more legible visualization, the grid \yafeng{normalized density} is then \mc{smoothed by a halo effect~\cite{oelke2011visual} where each grid is extended into a 5x5 grids, and we assign 30$\%$ density to the peripheral halo area}.
%When calculating the grid, the weight of the data points is determined according to the distance between the data point and the grid. The closer the distance is, the larger the weight is. The weight ranges from 0.4 to 1.0.
% \begin{equation}
%     \text{diff}_{i,j} = \sum_{|k-i| + |l - j| \leq 2}(\text{grid}^t_{k,l} - \text{grid}^{t-1}_{k,l})\cdot(1 - 0.3(|k-i| + |l - j|)).
% \end{equation}
% The density diff statistic of each grid aggregates the data of all grids with a Manhattan distance [ROSS: ADD "OF" ?] no more than two, and the weight of a grid to the aggregation decreases over longer distances. 
A positive value means the grid has a higher density in the \yafeng{latest streaming data} and is colored red.
A negative value means the grid has a lower density in the \yafeng{latest streaming data} and is colored in blue.
The darker the color, the higher the density difference. 
Fig~\ref{fig:first_year} shows an example of the density diff view.

\weikairevision{\noindent\textbf{Justification.} %The main goal of this view is to discourse the data distribution change. 
We considered using either a flow map or a sequence of screenshots to show the distribution change over time. However, we found that the flow map of the data distribution cannot support a detailed distribution analysis at a particular timestamp, and the screenshot sequence makes it hard to identify the %change of the distribution across different 
\lu{distribution change between}
screenshots~\cite{goldsberry2009issues}. Therefore, we adopted the streaming scatterplot because it can reveal the detailed distribution and support comparison~\cite{liu2016visualizing}. 
Analysts can switch between the \emph{scatterplot mode} and \emph{density diff mode}. We adopted this switching design because superposition can cause visual clutter, and juxtaposition would halve the view size and make it harder to investigate the distribution.
}

\subsubsection{Prediction-Level Visualization}
The prediction-level visualization consists of three views, a base learner view (Fig.~\ref{fig:teaser}D), a samples of interest view (Fig.~\ref{fig:teaser}E), and a performance view (Fig.~\ref{fig:teaser}F).

The \emph{base learner view} lists all available base learners that can be used in the ensemble model.
% One row describes one base learner, which is distinguished by an ID and a glyph pattern visual encoding.
\yafeng{For each base learner, it shows the size of the training set and the proportion of the data points in the training set that belong to each Gaussian component. 
This proportion is represented by a colored bar using the same color scheme in the streaming scatterplot.}
%In the GMM components column, a colored bar is used to show the percentage of each Gaussian component label of the training data.
%The color matches the colors used in the streaming scatterplot. 
Analysts can select a data subset to create a new base learner and choose which base learners to use in the ensemble model.\looseness=-1

\mc{The \textit{samples of interest view} is used to mark a subset of data as samples of interest, which can be revisited afterward.}
% As streaming data arrives, \yafeng{analyst can add the latest streaming data into his/her samples of interest list for performance checking and revisit.}
%batches of the stream are appended to the list of samples of interest. 
Similar to the base learner view, the colored bars show the percentage of Gaussian component labels in every batch.
To see the effect of each base learner on the samples, we calculate a model distribution and visualize it using the combination of each base learner's glyph pattern. 
%\weikai{
The model distribution is a summary of the importance of the base learners in making predictions for this dataset. 
\yafeng{The importance of each base learner is gauged by the sum of the weights every training sample takes from the base learner.}
%For each instance $x$ in the batch, we calculate the distance between the instance and base learners using $({x}-{\mu})^\intercal{\Sigma}^{-1}({x}-{\mu})$, where ${\mu}$ and ${\Sigma}$ is the mean and co-variance matrix of the training data of each base learner.
%We use softmax to transform the negative distance into weights, and then obtain the importance of each base leaner by summing over all data. %[These sentences need revise, and similar with the last paragraph of Sec.3]}
From the model distribution, the analyst can determine which base learner is important.
\weikairevision{We chose the table form here because it is simple and easy to understand~\cite{Muzammil2011DataAI}.}
%\weikairevision{We choose the table form to show the base learner list and samples of interest because it is simple and can serve our purpose, including adjusting the base learners and revisiting some interesting samples.}
%After each drift adaptation, the ensemble model is updated either by changing some of the base learners or updating their weights.
%Such an update will also be reflected by how these base learners affect these datasets. 

%The result of drift adaptation is reflected in the change of drift degree and prediction accuracy. 
%The drift degree is visualized on the drift degree line chart.
% and the streaming scatterplot.
The \mc{\textit{performance view} visualizes the model performance before and after adaptation to verify the effectiveness of drift adaptation.}
%This view is optional in practice because we do not require groundtruth labels for drift analysis and adaptation.
\yafeng{This view would only present on the data with labels.}
% \yafeng{Other than reflecting the effect of drift adaptation on the decrease of the drift degree, a more direct output is the change in model performance, which is important to our experts.}
To enable the exploration of prediction accuracy and visualize the direct effect of the adaptation, we utilize the design from Squares~\cite{ren2017squares} in our performance view, as shown in Fig.~\ref{fig:teaser}F.
\mcr{Squares is able to provide a compact and effective comparison between classifiers before and after adaptation.}
It shows each class in a column, which contains a vertical axis annotated by its class label. 
The left-most vertical axis indicates the prediction confidence ranges.
Summary statistics (true positive, false positive, and false negative) for each class are encoded in stacked bars along the corresponding axis. 
The length of the bar represents the percentage of data samples predicted with the corresponding confidence score.
Dark grey indicates true positive, light grey indicates false positive, and no-fill bars on the left of the axis indicates false negative. %\yafeng{[YAFENG: IF THE ABOVE SENTENCE IS NOT CLEAR, WE CAN USE THE FOLLOWING.]}
%Dark grey indicates true positive, which means this amount of samples are predicted correctly.
%Light grey indicates false positive, which means this amount of samples are predicted to be of this class but wrong.
%No-fill bars on the left of the axis indicates false negative, which means this amount of samples are predicted to be of another class but their true label is this class.
To see if the prediction performance has improved, the performance view can change into comparison mode to show the performance statistics of the latest model and the model prior to this adaptation.
%Ideally, we want to compare the performance on data in the future.
%However, this could only happen when the future data is acquired, as well as the labels.
%DrifVis supports model performance comparison on every data batch, and if this is explored after adding new data the performance is then reported regarding the future data relative to the time of the adaptation.
%if this is explored after adding new data the performance is then reported regarding the future data relative to the time of the adaptation.
%In comparison mode, the performance view shows two sets of parallel coordinates where the top one presents the statistics of the current model and the bottom one presents the statistics of the previous model.
% DrifVis supports model performance comparison on every dataset in the samples of interest list, and the train/test split is used to ensure the plausibility of the reported accuracy. 
%\yafeng{[How to interpret the lines?]}\weikai{[@lizhen. Also, I think it is changed a little since now we split train/test set. I will revise this two paragraphs tomorrow.]}


%In DriftVis, we use a straightforward method to decide the weights of base learners.
%The basic idea is that the more similar the test sample is to a base learner, the larger the weight should be.
%For each sample in the new [ROSS: I THINK WE NEED TO GO THROUGH THE DOCUMENT AND BE PRECISES ABOUT HOW WE REFER TO THE DATA, STREAMING vs. NEW vs. HISTORICAL, etc. DOCUMENT IS NOT CONSISTENT] data, we first calculate the similarity between the sample and the training data of each base learner as $s_i = -(x-\mu_i)^\intercal\Sigma_i^{-1}(x-\mu_i)$, where $x$ is the sample, $\mu_i$ and $\Sigma_i$ are the mean and co-variance matrix of the training data of the $i$-th base learner.
%Then, we apply softmax to the similarity vector $s = [s_1, ..., s_i,...]$ to normalize the weights of the base learners to $[0,1]$ with a summation equal to $1$. [ROSS: THIS SECTION ENDS VERY ABRUPTLY AND DOESN"T TIE INTO THE NEXT SECTION.]
% We can also obtain the weights of base learners on a batch of data by averaging the weights vectors.


\subsubsection{Coordinated Interactions}
DriftVis provides coordinated interactions among different views for drift analysis. 
When the analyst hovers over a data sample or selects a group of samples, the line chart will highlight the time (on the x-axis) when these samples occur.
The analyst can also brush the line chart to see the brushed samples highlighted on the scatterplot. 
The streaming scatterplot itself also possesses a rich set of interactions for data exploration.
In order to investigate data details, such as the feature values and raw data, the streaming scatterplot uses pop-up windows to display the information of hovered or selected data samples. 
%In scatterplot mode, the user can hover over a single instance to see its feature values or its textual content.
Lasso selection is supported to display a summary of the selected samples.
%In the density diff mode, hovering over a grid displays a summary of the instances falling in the nearby grids being used to calculate this diff. 
The streaming scatterplot also allows the analyst to hide Gaussian components when it is too crowded.
%in the scatterplot mode.
%Other than lining up the time and the scatterplot position of instances, streaming scatterplot is also linked with the base learners and samples of interest.

To decide which base learner to include in the ensemble, it is essential to know what data is used to train the base learner.
Hovering over a base learner highlights its training samples on the scatterplot, and if the analyst clicks on the base learner, these samples will be shown as selectable points so that they can be reused to train another base learner or be compared exclusively to the \yafeng{latest streaming data}.
%Similarly, data samples can also be revisited and explored by dataset in the samples of interest. 

%It is likely that when more drifts show up in the streaming data, more and more GMM components will be modeled and the view will become cluttered.
%As some components are constructed way before the current batch or the samples modeled in some components are not the interest of analysis, the user can click on the top-left legend to hide such components. 

Sometimes, an undesirable incremental GMM result may cause a false alarm on drift detection because some data are not compared with the closest distribution;
therefore, the drift degree is overestimated.
%, which leads to an overestimation when calculating the drift degree.
To reduce such false alarms, our system supports analysts to modify the incremental GMM result. %manually after investigating the data.
Analysts can select some data in the scatterplot and click ``Merge Component'' to confirm that these points should belong to \mc{one component. The belonging relationship of other data samples will be incrementally updated.}
% the ``target component'' -- the component with the largest proportion among the selected data.
% \yafeng{This update will trigger the recalculation of the GMM and eliminate the false alarm.}
%Since these points have updated the parameters of the GMM, for each selected data sample that is not in the target component, the tool not only changes its component but also reduces its effect on the original component and add its effect on the target component.










==> Analyzing Concept Drift in Streaming Data_2/5-application.tex <==
% !TEX root = EvoTree-KDD.tex
\section{Evaluation}
\label{sec:application}

\begin{figure*}[!t]
  \centering
{\includegraphics[width=\linewidth]{fig/weathercase/weather_1.pdf}}
{\rmfamily
\put(-465,2){(a) Sept. 1 to Sept. 15.}
\put(-287,2){(b) Oct. 1 to Oct. 23.}
\put(-111,2){(c) Oct. 24 to Nov. 2.}
}
  \vspace{-5.2mm}    
%\vspace{20mm}
%\caption{he streaming scatterplot shows the density change from summer to early autumn in 1949. The incoming data of each analysis period isindicated in the box.}
  %\caption{The streaming scatterplot shows the density change from summer to early autumn in 1949. In (a), the new data come (A) with lower temperature (B). In (b), a new component was detected (C). In (c), the new data come and deviated from the new component (D)}
  %R3Q6
  \caption{\weikairevision{The streaming scatterplot shows the density change from summer to early autumn in 1949:
  (a) the new data (A) came with a lower temperature (B);
  (b) a new component (C) was detected;
  (c) the following data (D) came and deviated from the yellow component.}}
  \label{fig:autumn_data}
   \vspace{-5.2mm}
\end{figure*}

% In this section, we present two case studies to demonstrate how DriftVis supports the identification, analysis, and correction of concept drift.

%R0Q1
\weikairevision{In this section, we conducted a quantitative experiment to evaluate the effectiveness of our drift detection method and then presented two case studies to demonstrate how DriftVis supports the identification, analysis, and correction of concept drift.}

\subsection{Quantitative Evaluation on Drift Detection}

%\noindent\textbf{Experimental settings.}
% \weikairevision{We \mcr{employed} the widely-used experimental setting in drfit detection~\cite{dasu2006information}.
% and simulated two datasets of data streams, $D_1$ and $D_2$.
% Each data stream consists of 5,000,000 data points, which are equally divided into 100 groups.
% $99$ drifts are then simulated by changing the data distribution from group to group.
% %Here we chose the $2$-D Gaussian distribution, while group $D_1$ varies the mean, and $D_2$ varies the standard deviation.
% \lu{The data in each group follows a $2$-D Gaussian distribution, while $D_1$ varies the mean, and $D_2$ varies the standard deviation.}
% %The data distribution varies from group to group and causes 99 drifts in each stream.
% %The data points in each group are drawn from a $2$-D Gaussian distribution, and the parameters of the Gaussian distribution vary from group to group.
% %Therefore, we simulated $99$ drifts in each stream.
% %We used two different streams groups, while group $D_1$ varies the mean and $D_2$ varies the standard deviation.
% We compare our method with three representative methods:  ITA~\cite{dasu2006information}, LDD-DIS~\cite{liu2017regional}, and TVD~\cite{webb2018analyzing}. 
% Since a large window size $w$ approximate the data distribution better, we set $w=10,000$ for all algorithms, and the other parameters are decided through a grid search process.
% To evaluate the performance, we classify the detected drift into four categories.
% For a drift happened \lu{at} $t$ and reported \lu{at} $t+\Delta t$, we say it is successfully \textit{detected} if $\Delta t<w$, \textit{late} if $\Delta t\ge w$ but reported before next drift happens, and \textit{missed} if not reported before \lu{the} next drift happens.
% \lu{A} \textit{false} drift happens if %the previous 
% \lu{a} drift is reported again before the next drift comes.
% Table~\ref{tab:result} reports the count of the four categories averaged on 10 trails.
% %We report the average result on streams generated with ten different random seeds for each group \lu{in Table~\ref{tab:result}.}
% }
%\noindent\textbf{Results.}
% Table~\ref{tab:result} reports the count of the four categories averaged on 10 trails.
% \weikairevision{%Table~\ref{tab:result} 
% \lu{It} shows our algorithm achieves the highest true detection number and lowest late/miss rate in both groups, while the false alarms rate is lower in $D_1$ and comparable in $D_2$.
% This result implied that our method is more sensitive.\looseness=-1}


\noindent \textbf{Experimental setting.} \mcr{We \mcr{employed} the widely-used experimental setting in drift detection methods~\cite{dasu2006information,FengGu2016}.
Two synthetic datasets, $D_1$ and $D_2$, were used.
Each dataset consists of 5 million data points, which follow $2$-D Gaussian distributions.
There are $99$ simulated concept drifts in each dataset.
The drifts were simulated by changing the mean and variance of the Gaussian distributions in $D_1$ and $D_2$, respectively.
We compared our method with three baseline methods: ITA~\cite{dasu2006information}, LDD-DIS~\cite{liu2017regional}, and TVD~\cite{webb2018analyzing}.
In our experiment, we used a grid search to obtain the best hyper-parameters.}

\noindent \textbf{Criteria and results.} \mcr{
We classified the detected drifts into four categories by comparing them with the ground-truth.
When a drift happens \lu{at} $t$ and is reported \lu{at} $t+\Delta t$, the drift is considered to have been successfully \textit{detected} if $\Delta t<w$, \textit{late} if $\Delta t\ge w$ but is reported before next drift happens, and \textit{missed} if it is not reported before \lu{the} next drift happens. Here, $w$ is the window size of the respective method.
\lu{A} \textit{false} alarm happens if %the previous 
\lu{a} drift is reported again before the next drift occurs.
In practice, we want to maximize the number of \textit{detected} drifts and minimize the other three categories.
Table~\ref{tab:result} shows the number of drifts in each category for each method.
To reduce randomness, we reported the numbers averaged over 10 runs.
Compared with the baselines, our method has detected the largest number of \textit{detected} drifts in both datasets, demonstrating an improvement over existing drift detection methods.
However, we noticed that, compared with $D_1$, our method performed worse in $D_2$.
The potential reason is that the energy distance mainly focuses on the mean ($D_1$) of the distribution instead of the variance ($D_2$).\looseness=-1
}

\begin{table}[!t]
\vspace{-0.5mm}
\caption{Comparison of drift detection results.} 
\vspace{-1mm}
%\setlength{\tabcolsep}{3.5mm}{
\begin{tabular}{clcccc} 
\toprule 
Dataset & Method & Detected & Late & Missed & False \\ 
\midrule 
\multirow{4}*{$D_1$} & ITA~\cite{dasu2006information} & 75.5 & 12.3 & 11.2 & 4.5 \\
~ & LDD-DIS~\cite{liu2017regional}& 56.5 & 19.3 & 23.2 & 3.9 \\
~ & TVD~\cite{webb2018analyzing} & 75.5 & 19.9 & 3.6 & 7.0 \\
~ & Ours & \textbf{97.9} & \textbf{0.9} & \textbf{0.2} & \textbf{0.8} \\
\hline
\multirow{4}*{$D_2$} & ITA~\cite{dasu2006information} & 75.7 & 18.0 & \textbf{5.3} & 7.6 \\
~ & LDD-DIS~\cite{liu2017regional} & 44.0 & 22.2 & 32.8 & 12.2 \\
~ & TVD~\cite{webb2018analyzing} & 71.2 & 22.3 & 5.5 & \textbf{6.0} \\
~ & Ours & \textbf{77.5} & \textbf{14.9} & 6.6 & 6.4 \\
% I made a mistake in the parameter between different seeds... The system update automatically before the experiment finish, and I continue the experiment with following seeds, but the parameter is changed - -!
%~ & Ours & \textbf{81.0} & \textbf{12.9} & \textbf{5.1} & 6.8 \\
\bottomrule
\end{tabular}
\label{tab:result}
\vspace{-5mm}
%}
\end{table}

\subsection{Case Study}

\subsubsection{Tabular Data: Weather Prediction}

\noindent\textbf{Dataset}.
This dataset is compiled by the U.S. National Oceanic and Atmospheric Administration (NOAA).
We use a preprocessed subset that has been used in previous concept drift detection research~\cite{ditzler2012incremental,elwell2011incremental}.
It contains 18,159 daily weather records from the Offutt Air Force Base from 1949 to 1999.
Each weather record contains eight measurements (``Temperature,'' ``Dew Point,'' ``Sea Level Pressure,'' ``Visibility,'' ``Average Wind Speed,'' ``Maximum Sustained Wind Speed,'' ``Maximum Temperature,'' and ``Minimum Temperature'') and one class label (``precipitation'').
In our analysis, we predict whether rain precipitation was observed on each day.
%precipitation includes rain alone, snow alone, and a mix of the two.
For the prediction model, we use logistic regression implemented in Scikit-learn 0.21.3.
We randomly split the dataset into 70\% training and 30\% test data.
The training/test split is used to ensure the plausibility of the reported accuracy.
% \mc{Compared with the second case study on textual data ($60\%$ training and $40\%$ testing), we use 10$\%$ more data samples for training because we found that if we used less data, there was a serious over-fitting problem.}

\noindent\textbf{Drift analysis}.
We conducted this case study together with E$_1$, our expert from the China Meteorological Administration. 
She works on weather prediction model development and making weather prediction decisions.
In this case, we first illustrate how DriftVis helped identify changes in the weather data distribution across seasons, and then demonstrate how it facilitated the expert in identifying abnormal weather changes long-term.
\lu{This study will show that a high drift degree could be detected when the data sees a new season, but DriftVis could also find small drifts before the drift degree reaches an alert level.}
 
\noindent\textbf{Seasonal drifts in the first year.}
The initial model, $BL_0$, was trained on data from the summer of 1949 (June 1 to August 31). 
The remainder of the data was used to simulate a streaming context, where data is reported daily. 
When E$_1$ saw a drift, she stepped in to analyze.
The drift degree first went up to 0.2 after 15 days, on Sept. 15, and the expert decided to explore the data distribution change.
In Fig.~\ref{fig:autumn_data}(a), she found that these new data were on the boundary of the existing component with relatively lower temperature, as shown in Fig.~\ref{fig:autumn_data}A and Fig.~\ref{fig:autumn_data}B.
%\ross{[ROSS: In Figure 4, how can I tell that these are lower temperature?]}
She selected the new data and some similar data points from the historical data to build a new base learner, $BL_1$, and combined $BL_1$ with $BL_0$ to create a new ensemble prediction model.
After the adaptation, the drift went down, indicating that the adaptation was successful.\looseness=-1
%\mc{There was a similar pattern on Sept. 30 where the drift degree increased to 0.2.
%It triggered E$_1$ to replace $BL_1$ with a new base learner ($BL_2$), which contained the new data and the training data in $BL_1$.}\looseness=-1
%The data kept streaming in and the drift degree increased to 0.2 after another 15 days, on Sept. 30.
%These 15 days weather data projected close to the previous 15 days data. % (Fig.~\ref{fig:autumn_data}(b)).
%The expert commented that September was the start of autumn and the temperature dropped.
%\yafeng{[LOOK AT STATISTICS SUMMARY to see why you want to use BL2 to replace BL1]}
%She enlarged the training set of BL1 by adding these new data and replaced BL1 with a new base learner (BL2).

\mc{Since Oct. 1, there were some data samples deviating from the blue component, and on} Oct. 23, the expert identified a new Gaussian component (yellow, as shown in Fig.~\ref{fig:autumn_data}C) in the streaming scatterplot (Fig.~\ref{fig:autumn_data}(b)). 
The expert explained, ``This is the first month of autumn, and the temperatures have begun \mc{to} decrease.
This is why a new component has emerged.''
However, she commented that the drift degree was still low, and many points in the yellow component were flipped from the blue component. % and had also been covered in BL2.
Therefore, she decided to monitor the change closely for the following days.
As expected, the next few days' data all fell into the yellow component, and the expert noticed an increase in drift degree, which went up to 0.2 on Nov. 2.
Fig.~\ref{fig:autumn_data}(c) shows the corresponding streaming scatterplot and Fig.~\ref{fig:autumn_data}D highlights where the latest streaming data appeared. 
E$_1$ created a base learner ($BL_2$) using the yellow component data and removed $BL_1$.
She explained, ``This component does not have a full collection of autumn data yet, but in our field, we always want to adapt the model to create a better prediction as soon as we have enough data.
While we know that when more autumn data comes in, the data pattern learned using this subset may not be robust, further adaptation can always be made.''
Just as the expert explained, the drift degree stayed low for the next few days because the model learned some patterns from the yellow component, which encapsulates many properties of the incoming data.
%\mc{On Nov. 19, the drift degree increased to 0.2.
%As same as $BL_2$, E$_1$ replaced $BL_3$ by a new base learner $BL_4$ to include more autumn data.}
%However, the drift degree went up to 0.2 again on Nov. 19, late autumn.
%The expert noted that late autumn has obviously lower temperatures than the previous data. 
%Therefore, she removed BL3 and created BL4 by including more autumn data.
%Selecting all data samples in the yellow component, our expert created a new base learner (BL4) and removed BL3.
%The drift degree stayed low since then for a couple of weeks and the new streaming data were projected into the yellow component.
%At this time, our ensemble model had two base learners, BL0 and BL4.
%BL0 was trained on the initial 90 days of the summer.
%BL4 was trained on the yellow component data most of which were autumn data.

\begin{figure}[b]
  \centering
   \vspace{-3mm}
{\includegraphics[width=\linewidth]{fig/weathercase/weather_2.pdf}}
{\rmfamily
\put(-242,2){\textls[-5]{\spaceskip=0.16em\relax(a) A component built on Dec. 11.}}
\put(-117,2){\textls[-5]{\spaceskip=0.16em\relax(b) A component built on Jan. 31.}}
}
\vspace{-5.5mm}
  %\caption{The streaming scatterplot shows the distribution change in the winter of 1949. The box indicates where the expert investigated. }
  %R3Q6
  \caption{\weikairevision{The streaming scatterplot shows the distribution change in the winter of 1949:
  (a) the appearance of the green component (A);
  (b) the purple component (B) was built, which shared a similar pattern to the green component, e.g., low temperature and high sea level pressure (C).}}
  \label{fig:winter_data}
   %\vspace{-4mm}
\end{figure}



% \mc{Similar to autumn, since Nov. 20, there were some data samples deviating from existing components and on}
On Dec. 11, a green component (Fig.~\ref{fig:winter_data}A) appeared, and on the same day, the drift degree increased rapidly to 0.15.
%was also up to 0.2. 
Similar to how she handled the occurrence of the yellow component, the expert first built a new base learner ($BL_3$) with available data in early winter and replaced it with $BL_4$ once the green component had more data and the drift degree increased.
%Although the green component only had a few data points, the expert wanted to update the model so that these new data in early winter can be covered.
%She selected all data from the new component and some other data points projected closely to build a new base learner (BL5).
%The reason for selecting more data than purely the new component’s data was to avoid overfitting.
%Similar to first adding base learner BL2 when the yellow component occurred, BL5 may not be able to fully explain the data distribution of the green component because it just emerged and will grow as more winter data comes in.
%The data points of the next 15 days all fell into the green component except one day and the drift degree increased to 0.2 gradually.
%\yafeng{[FIG: scatterplot and linechart]}
%Using all data in the component, our expert built a new base learner BL6 and replaced BL5.
%More winter data streamed in and the drift degree didn't go up until 10 days later.
%Our expert saw the drift degree started to increase and approached 0.2 on Jan. 8 1950.
%Most of these 13-day data belonged to the green component.
%Using all data in this component, the expert created base learner BL7 and used it to replace BL6.
%Similar to previous adjustment, the expert replace BL6 with BL7 which include all data in the green component.
As of Jan. 8, 1950, the ensemble model had three base learners, $BL_0$, $BL_2$, and $BL_4$.


\begin{figure}[b]
  \centering
   \vspace{-4mm}
\subfigure%[The density diff between the spring and previous data.]
{\includegraphics[width=\linewidth]{fig/weathercase/weather-3.pdf}}\\
\vspace{-4mm}
  \caption{Exploring the density change of the yellow component. The left figure shows the scatterplot on May 31, 1950, and the right figure shows the density diff comparing the latest streaming data to the training data of $BL_2$ (yellow component).}
  \label{fig:first_year}
%   \vspace{-4mm}
\end{figure}

In late January, the weather became very cold, and a fourth Gaussian component (purple, Fig.~\ref{fig:winter_data}B) appeared on Jan. 31, as shown in Fig.~\ref{fig:winter_data}(b).
%\yafeng{[FIG: scatterplot Jan. 31, show feature stats.]}
At this time, the drift degree was not high, and %but the expert saw that the purple component was not covered by historical data distribution and wanted to update the prediction model to include these data.
\weikai{E$_1$ commented that these data in purple shared a similar pattern to the green component, e.g., low temperature and high sea level pressure, as illustrated in the line chart in Fig.~\ref{fig:winter_data}C}.
Based on this observation, she merged the purple component into the green component and used all of the data in the green component to create a new base learner $BL_5$ and replaced $BL_4$. % (Fig.~\ref{fig:winter_data}(c)).
%The drift degree was below 0.2 all the way to the end of May when DriftVis had explored a full year of the weather data.
%However, the expert decided to adjust the model covering the yellow component because she saw density increased in some region regarding this component.

The drift remained low for the following two months but went up again in early April, when the expert noticed a few days with relatively higher sea level pressure for the time in a year. 
The drift degree increase was a false alarm caused by a mis-clustering of the incremental GMM, and the expert corrected this by merging these points into the green component. 
By the end of the first full year, E$_1$ decided to adjust the model covering the yellow component because she saw density increased in some regions in this component.
\yafeng{Comparing the latest streaming data with the training data in $BL_2$, which was built on the yellow component earlier, Fig.~\ref{fig:first_year} shows that in the area of the yellow component, there were some red grids in the density diff mode. 
This indicated that the latest streaming data in the yellow component were likely to have a different density distribution than what had been modeled. Specifically, the area with deep red grids became denser.} 
%Fig.~\ref{fig:first_year} shows a few red regions in which the density increased.
%She commented that having the data of four seasons would be important for a weather prediction model, and she would feel more comfortable if the model could be improved when we have just finished exploring the first year.
Therefore, using a new base learner $BL_6$ trained on all data in the yellow component, E$_1$ replaced $BL_2$.
The current model ($M_1$) now includes base learner $BL_0$, $BL_6$, and $BL_5$, and the model accuracy running over the past year is 0.77.\looseness=-1
%\weikai{The current model achieved 0.76 accuracy over this year.}
%\yafeng{[MODEL 1 with acc]}



\noindent\textbf{Occasional drifts after having four seasons.}
When it came to the second summer (1950), the drift degree stayed under or around 0.1 until July.
E$_1$ wanted to explore the data at the end of June because she saw some yellow points were projected in the blue density area (Fig.~\ref{fig:extreme_high_temp}).
Looking at the feature values of these yellow points, she found that these days had high max temperatures ($\sim95^{\circ}F$) and low sea level pressures ($<1006$).
She commented that these days could be extreme days in the summer when compared to the historical data.
It was more reasonable to group them into the blue component, which includes the data of last summer than associating them with the yellow component, which had typically autumn and spring data.
She merged these yellow points into the blue component and replaced $BL_0$ with a new base learner $BL_7$ using the refined blue component. 
The drift degree became lower.

\begin{figure}[!tb]
  \centering
%   \vspace{-3mm}
%\subfigure[The scatter plot after first year..]
{\includegraphics[width=0.9\linewidth]{fig/weathercase/weather-4.pdf}}
\vspace{-3mm}  
  \caption{The yellow points in the blue region show high max temperature and low sea level pressure and are more similar to summer data (blue component) than autumn data (yellow component). }
  \vspace{-5mm}  
  \label{fig:extreme_high_temp}
   \vspace{-1mm}
\end{figure}

%In the following days, the samples of interest view showed that most of the data were in the blue component, and the corresponding base learner $BL_7$ was reused.
%The drift degree increased in mid-September 1950, and E$_1$ then analyzed the data.
%\weikai{While she did not see these days were projected outside of existing density areas, the expert examined the density diff and found some red grids in the blue component.
%The corresponding data had small temperature differences between day and night.
%Seeing this as a new pattern which might affect the precipitation, she built a base learner $BL_{8}$ using all current blue component data and replaced $BL_7$.}
After exploring the weather data for more than 14 months, the data had been relatively well covered by the model, and the drift degree stayed lower than 0.1 for the remainder of 1950 and the following year.
This model ($M_2$) comprises $BL_8$, $BL_6$, and $BL_5$. 
While more weather data streamed in, the expert conducted two more adaptations in 1952 in mid-July and mid-September, respectively, updating base learners and creating a model ($M_3$) with $BL_{9}$, $BL_{10}$, and $BL_{5}$. \looseness=-1
%Afterwards, the ensemble model (M3) uses BL8, BL12, and BL13, 
%and there were no drift for the following two years. 
%\yafeng{[MODEL 3 with acc]}

Comparing the precipitation prediction accuracy of the three models with their last adaptation in Jun. 1950 ($M_1$), Sept. 1950 ($M_2$), and Sept. 1952 ($M_3$), we run them on yearly test data from Jun. 1949 to May 1954. $M_1$ has its yearly accuracy being 0.77, 0.72, 0.73, 0.67, and 0.74; $M_2$ has its yearly accuracy being 0.78, 0.74, 0.73, 0.69, and 0.76; and $M_3$ has its yearly accuracy being 0.79, 0.75, 0.76, 0.73, and 0.81.
Their prediction accuracy shows that with further adaptations, $M_2$ performs better than $M_1$, and $M_3$ is even more accurate than $M_2$, especially in the fourth and fifth years. 
% The improvement on the prediction accuracy also indicates that DriftVis is effective at supporting analysts in identifying and overcoming drift. 
The improvement of the prediction accuracy also indicates that DriftVis is effective in identifying and overcoming drift. 



\subsubsection{Textual Data: Academic Paper Topic Evolving}
\begin{figure*}[!tb]
  \centering
%   \vspace{-3mm}
\subfigure[\yafeng{Exploring} papers from 2000 to 2003.]
{\includegraphics[width=0.44\linewidth]{fig/textcase/t1.pdf}}
\hspace{0.05\linewidth}
\subfigure[\yafeng{Exploring} papers from 2004 to 2007.]
{\includegraphics[width=0.44\linewidth]{fig/textcase/t2.pdf}}\\
\vspace{-3mm}
\subfigure[\yafeng{Exploring} papers from 2008 to 2011.]
{\includegraphics[width=0.44\linewidth]{fig/textcase/t3.pdf}}
\hspace{0.05\linewidth}
\subfigure[\yafeng{Exploring} papers from 2016 to 2018.]
{\includegraphics[width=0.44\linewidth]{fig/textcase/t5_2.pdf}}\\
\vspace{-3mm}    
%\vspace{20mm}
  %\caption{\yafeng{The scatterplot shows the Gaussian components in different years when analyzing NeurIPS papers. Each subgraph shows the different analytics steps our expert took and illustrates the interesting components explored.}}
  %R3Q6
  \caption{\weikairevision{The scatterplot shows the Gaussian components in different years when analyzing NeurIPS papers. Each subgraph shows the different analytics steps our expert took. The regions (A)-(K) indicates the interesting components explored.}}
  \label{fig:text}
   \vspace{-4mm}
\end{figure*}

% We use the academic papers in the textual case here.
% Since , the distribution of the papers is actually changed gradually.
% For example, the SVM and kernel methods are hot at the beginning of the 21st century and then cool down gradually, while the neural network is catching more and more attention.

%There are dynamic changes in the topics of academic papers over the years, which may induce concept drift.
% In this case, we focus on detecting, analyzing and adapting a multiclass text classification model to potential concept drift.

\noindent\textbf{Dataset.}
This dataset consists of 7,926 papers from the top-tier machine learning conference, NeurIPS (from 2000 to 2019).
% We use the first four year
% These papers were split into 5 batches, where each batch contains papers from a consecutive 4 years time span 
% [ROSS: WHY DIDN'T WE DO THIS YEARLY? JUST TRYING TO REMEMBER.].[One reason is that the change of the topics is very slow, another reason is to make the case shorter.]
% is aggregated into a data batch.
% For each paper, we used its title, abstract, and introduction and further preprocessed the abstract by tokenization, lemmatization and discarding noisy words [ROSS: GIVE EXAMPLES OF NOISY WORdS AND HOW WE DETECTED THEM?]. 
For each paper, we extracted the title, abstract, and introduction and further preprocessed \yafeng{the text} by tokenization, lemmatization, keeping only the top-5000-most frequent words in the corpus. 
% crawled the papers from NeurIPS from 2000 to 2019 and used the text in to represent each paper.
% Such words were determined by building a dictionary of top-5000 frequent words over the whole corpus, and words not belonging to this dictionary is considered as low-frequent words.
Each paper was then converted into a 5,000-dimension vector, and each dimension was reweighted \yafeng{using the TF-IDF scheme}~\cite{manning2008introduction}.
% [ROSS: ADD A CITATION HERE FOR COMPLETENESS]
% After some necessary natural language processing such as tokenization and lemmatization, we keep the words that have top-5000 frequency and then convert the text of each paper into a vector of words.
% Then we use the widely to increase the weights of the rear words. 
To accelerate the computation of the constrained t-SNE, we further reduced the dimension of each paper to $10$ by singular value decomposition (SVD).
%The reason why we utilize this dimension reduction algorithm is that each dimension in SVD is more interpretable since how much each word contributes to it is known.
\yafeng{The reason for using SVD is that the contribution of the words can be interpreted intuitively from each reduced dimension.}

% However, we cannot use this word vector as the input directly because of its high-dimension and sparsity.
% To embed these vectors into low-dimension space, we performed to reduce the dimension.
% This technique is also known as a typical method of Latent Semantic Analysis (LSA) in the natural language processing field.

In this case, we collaborated with E$_3$ to explore the prevalent research topics in NeurIPS.
To \mc{help E$_3$ gain insights from the past research}, we built a multi-class text classifier that predicted the topic of a paper.
To get the ground-truth label for each paper, we employed a ten-topic Latent Dirichlet Allocation~\cite{blei2003latent} to calculate the topic distribution of each paper.
Each paper's initial ground-truth label was set to the most dominant topic in the topic distribution.
We further invited E$_4$ to verify and fine-tune the ground-truth labels of ambiguous papers with mixed topics.
Given the ground-truth labels, we built an SVM-based 10-class classifier to predict the label (topic) of each paper. 
% to adopted the widely-used Support Vector Machine (SVM) as the classifier to 
% [ROSS: WHY DID WE SWITCH FROM LDA TO SVM?]
% [\weikai{Weikai: LDA helps generate labels and create a classification task. We use SVM for classification.}]
\mc{We randomly split the dataset into $60\%$ training and $40\%$ test data.
The training/test split is used to ensure the plausibility of the reported accuracy.
We used the training papers in 2000-2003 to build an initial model, whose accuracy was $0.75$.
The papers after 2003 were assumed to stream in year by year to simulate the common practice of E$_3$, where he went through the NeurIPS papers after each year's conference to discover emerging topics and trends.\looseness=-1}
 
% The training data is set as $60\%$ of the papers in the first four years (2000-2003).
% The accuracy of the remaining $40\%$ %of the papers in these four years 
% was $0.75$.

% \mc{For drift adaptation and performance evaluation, these papers were also split into $60\%$ training data and $40\%$ test data.
% As same as the case study on weather prediction, }
% and the other papers are the streaming data, which are processed yearly.} 
% $60\%$ papers from the the first batch are used as the training data and the remaining papers were used as the test data.

% of papers is randomly split into training/test set with the ratio of $60\%/40\%$.

% so that the accuracy after the adapation in the current batch is also meaningful.
% we first used a ten-topic to calculate the distribution of topics for each document.
% The most of the labels are set to the most dominant topic, and the expert helped to refine the labels of some documents with .
% For the classifier, we used because of its success on text classification tasks.
% We use Natural Language Toolkit 3.4.5 for the natural language processing and Scikit-learn 0.21.3 for computing the word vectors, reducing the dimension, and building the SVM classifier.

\noindent\textbf{Analysis of papers in 2000-2003.} 
E$_3$ started the analysis with the papers in 2000-2003 (754 papers).
Fig.~\ref{fig:text}(a) shows the distribution of these papers.
Several topics were identified from this distribution by hovering over the papers in the scatterplot to examine the keywords and titles. 
% We selected the points in each component and quickly identified several topics with the help of the displayed .
For example, the keywords in the green component (Fig.\ref{fig:text}A) were ``kernel, vector, feature.''
E$_3$ commented that there was a high research interest in the kernel methods at that time due to the success of support vector machines, which was reflected in the leader-board of the MNIST dataset~\cite{MNIST_lb}.
% The light blue component ($\#0$) was mainly about graphical model and Bayesian learning.
The orange component ($\#5$) contained two inner clusters (Fig.\ref{fig:text}B and C).
% topics and can be visualized in the scatterplot.
The \yafeng{top} one (Fig.\ref{fig:text}B) focused on neural networks, while the bottom one (Fig.\ref{fig:text}C) focused on reinforcement learning.
%\yafeng{E$_3$ expected these two inner clusters to split if their respective topics become popular in the future.}
E$_3$ commented that these two inner clusters might split if their respective topics become popular in the future.\looseness=-1
%E$_3$ was interested in why papers of two different topics \yafeng{were} merged into one component.
%After checking the titles of these papers, he found that the two sets of papers \yafeng{were} assigned to one component because they each consisted of a small number of papers.
% \mc{I dont buy in the explanation of ``the bottom one tended to be a new component but currently combined with the left one due to its insufficient size.''}
% \weikai{[These papers are just assigned to this component temporarily because the component size is small. When more papers come it will splitted.]}

% As a baseline, we trained the classifier as mentioned before by splitting the batch into \weikai{460/294 (roughly 0.6:0.4).}


\noindent\textbf{Analysis of papers in 2004-2007.}
Next, the papers from 2004 to 2007 were added year by year.
In the year 2007, the drift degree increased to 0.15 and triggered E$_3$'s detailed analysis.
% We noticed that the drift increased to 0.15.
% gradually\mc{where is the figure??}. \weikai{[I do not put the figure here because currently all figure in Fig.7 is about scatterplot, and insert a line chart may look weird. Also I think that use a line chart to explain a value seems a little 'wasty'. Now I upload the line chart in fig/textcase]}
As shown in Fig.~\ref{fig:text}(b), he found that there were three new components compared with the training data (2000-2003).
In particular, component $\#8$ (Fig.~\ref{fig:text}D) \yafeng{separated} from the previously mixed component $\#5$ (Fig.~\ref{fig:text}B and C) because it now had a sufficient number of papers to form a new component.
% The papers about `spike' and neuron' from the old component ($\#5$).
%We also found that some red points (\mc{figure}) are projected away from the main component.
% previous region of the reinforcement learning component.
%These papers were found to have focus on ``regret'', \mc{which was a rising topic at that time.}
% Such an approach differed from the main cluster, where 
% which differed from the words like ``policy.''
% \mc{Not finished this part, I cannot link the color to the cluster} 
The pink component (Fig.~\ref{fig:text}E) talked about convex optimization.
% which had gradually increased in popularity.
The keywords in the brown component (Fig.~\ref{fig:text}F) were ``latent'' and ``topic.'' 
This new component appeared due to the success of Latent Dirichlet Allocation~\cite{blei2003latent}, which was published in 2003.\looseness=-1
%\yafeng{Other than finding the new components, E$_3$ also found that} \mc{there were some papers in the green component deviating from the existing components (Fig.~\ref{fig:text}F).}
% the left part of the green component ($\#2$) also grew gradually (Fig.~\ref{fig:text}(b)(F)).
%\mc{These papers were about spectral clustering~\cite{ng2002spectral} with keywords ``matrix,'' ``manifold,'' and ``spectral clustering.''}
% The topics were now focusing on 
%The expert confirmed that spectral clustering was popularized in the machine learning field by one fundamental paper~\cite{ng2002spectral} published in NeurIPS 2002.\looseness=-1

Since there were three new components and a relatively large drift degree of $0.15$, the expert decided to build new base learners to adapt to this drift.
%The papers in these three new components (227 papers) were chosen to train three new base learners (SVM), respectively.
Using the base learner view (Fig.~\ref{fig:teaser}D), the expert selected the papers in these three components and built three base learners with the papers in the components.
After merging these three new base learners and the old one into an ensemble model (Sec.~\ref{sec:system}),
\mc{the drift degree decreased from $0.15$ to $0.07$, and the \weikairevision{classification} accuracy improved from \textbf{0.73} to \textbf{0.75} \liu{in the papers published during 2004-2007}.\looseness=-1}

%\noindent\textbf{Analysis of papers in 2008-2011.}
%As papers from 2008-2011 were added, the drift degree slowly increased to $0.10$, which
% over time was slower than that in 2004-2007
%indicated the relatively slow development of novel topics in the machine learning community prior to the deep learning era.
% which indicated no large topic change in the machine learning community at that time period.
% After the above adaptation, the increase of the drift degree over years was slowed down (\mc{A line chart comparison here}), showing the effectiveness of the adaptation.
%To verify this assertion, the expert performed a detailed examination after he \yafeng{added} the papers in the year 2011. 
% In the years 2008-2011, the drift degree remained relative low ($<0.1$).
% To verify that there was no large topic change, the exper
% and increased to \mc{0.14} and triggered E$_3$ to perform the second examination.
% remains low in the next a few years (2008-2011) and gradually increased to .
% It indicated that there is not as much topic changes as the in 2004-2007.
% In the exploration, the expert examined the visualization at the year 2011 to verify this.
%As shown in Fig.~\ref{fig:text}(c), there were no new components formed. %since 2007.
%Nevertheless, he still found minor drift in the components by examining the keywords.
%For example, in the pink component (Fig.~\ref{fig:text}G), there were some papers noticeably deviating from the existing component.
%Compared with the other papers in this component, these papers had new keywords ``lasso,'' ``regularization,'' and ``low-rank.'' 
% These papers were about sparse optimization, like the widely-used LASSO~\cite{tibshirani1996regression}.
%LASSO~\cite{tibshirani1996regression} was a widely-used optimization technique that could date back to the 1990s.
%The expert was curious why such a technique gained research attention again.
% After checking the corresponding papers, he found that the L1 regularization in LASSO was able to produce a sparse coding of an input signal, e.g., an image.}
% In 2006, there was a breakthrough in the sparse coding in signal processing~\cite{candes2006robust}.
%After checking the corresponding papers, he found that because of a breakthrough in using a sparse coding in signal processing in 2006~\cite{candes2006robust}, many researchers started to use the L1 regularization in LASSO to produce the sparse coding.
%As a result, LASSO attracted much attention in the next few years.
% One representative work is the widely-used LASSO~\cite{tibshirani1996regression}.}
% E$_3$ commented that this popularity of sparse optimization, e.g., LASSO~\cite{tibshirani1996regression}, was mainly triggered by the 
%As there was only minor concept drift, the expert decided not to update the model.

% here is the original text from a survey in 2013 "Submodular Function Maximization"
% It appears in a wide variety of applications: in Computer Science it has recently been identiffed and utilized in domains such as viral marketing (Kempe et al., 2003), information gathering (Krause and Guestrin, 2007), image segmentation (Boykov and Jolly, 2001; Kohli et al., 2009; Jegelka and Bilmes, 2011a), document summarization (Lin and Bilmes, 2011), and speeding up satisffability solvers (Streeter and Golovin, 2008). 
% See (Fujishige, 2005) and (Schrijver, 2003) for an in-depth discussion of submodular functions and their properties. This chapter focuses on modern results on submodular maximization. There has been extensive research into algorithms for minimizing submodular functions (c.f., Fujishige 2005; Schrijver 2003).
% Fujishige, Satoru. 2005. Submodular functions and optimization. 2nd edn. Vol. 58. North Holland, Amsterdam: Annals of Discrete Mathematics.
% Schrijver, Alexander. 2003. Combinatorial optimization : polyhedra and efficiency. Volume B, Part IV, Chapters 39-49. Springer.


% 0425 ------
% There is a great increase of density in the middle (Fig.~\ref{fig:text}(E)) of the optimization component ($\#6$) because \weikai{many papers focus on ``submodular minimization'' to solve some computer science problem, such as graph cuts after Fujishige discussed this topic in his book~\cite{fujishige2005submodular}}.
% The density of the right part of the component (Fig.~\ref{fig:text}(E)) also increased a lot.
% The papers contained keywords of ``low-rank'' and ``sparse'', which were paper on sparse optimization, like the widely-used LASSO~\cite{tibshirani1996regression}.
% Expert E$_3$ commented that this trend was mainly triggered by the breakthrough in the sparse coding in signal processing~\cite{candes2006robust}.
% As expected, the brown component ($\#7$) on latent variables kept growing (Fig.~\ref{fig:text}(F)).
% In the reinforcement learning component ($\#8$), there were lots of papers that were not covered by the previous papers (Fig.~\ref{fig:text}(G)), and ``bandit'' was their keywords.
% Bandit problem first appeared in the NeurIPS conference in 2005.
%--------0425------


% The increasing attention was driven by potential applications in structured decision making in dynamic environments, such as network routing, path planning, and job scheduling.
% As a result, a new topic about bandit was formed in the NIPS paper corpus.
% As there was only minor concept drift, the expert decided not to update the model.
% \weikai{[Or 2007 is better? See the list in comments.]} \mc{where is the list...}\weikai{[It is commented in the source text.]}
% Nearly tight bounds for the continuum-armed bandit problem 2005
%The Price of Bandit Information for Online Optimization 2007
%The Epoch-Greedy Algorithm for Multi-armed Bandits with Side Information 2007
%Structure Learning in Human Sequential Decision-Making 2008
%Online Optimization in X-Armed Bandits 2008
%Mortal Multi-Armed Bandits 2008
%An Online Algorithm for Maximizing Submodular Functions 2008
%Algorithms for Infinitely Many-Armed Bandits 2008
% Later, around 2008, NeurIPS authors paid more attention to this topic.

% We also examined whether the adaptation in the previous batch helped the classification in this batch.
% The accuracy of the initial model was 0.63 (trained on the first batch), while the adapted one was 0.76 (trained on the first batch and papers from the three new components).

\noindent\textbf{Analysis of papers in 2012-2015.}
% We further added papers from 2012 to 2015 (1,542 papers) and found no new components are detected.
% After 1,542 were added, although there is still no new component formed, the drift was still gradually increasing, and we can also found more drift on the scatterplot.
The drift degree increased gradually from 2012 to 2015.
In 2015, the drift degree increased to 0.14, and it prompted
E$_3$ to perform an analysis of this drift.
This drift was expected because E$_3$ knew that these years were the dawn of the deep learning era, and new machine learning approaches were developed.
% It is expected by the expert
% Similar with the previous batch, there were some drift in the existing components.
He found that no new component was formed, and there were no deviating data samples.
Thus, E$_3$ switched to the density diff mode to further examine the root cause of the drift.
He found that 
% the keywords in the components greatly changed due to the development of deep learning.
the most noticeable drift happened in the pink component ($\#6$), where the density of three regions increased (Fig.~\ref{fig:teaser}G, H, and I).
% As there were no new components or deviating samples, the expert switched to the density diff mode.
% As shown in Fig.~\ref{fig:teaser}, the density increased in two regions of the pink component. 
The left-top part of the pink component (Fig.~\ref{fig:teaser}G) was about deep neural networks, which was a rising topic at that time.
E$_3$ commented that this new topic was triggered by AlexNet~\cite{krizhevsky2012imagenet} being the winner of the ILSVRC2012 image classification challenge.
% The network achieved a top-5 error of 15.3$\%$, 10.8$\%$ lower than that of the runner up.
% As a proof of influence, the corresponding paper got more than 50k citations.
The bottom part of the pink component (Fig.~\ref{fig:teaser}H) was about variational inference.
This topic became popular due to the introduction of an efficient deep generative model - Variational Auto-Encoder (VAE)~\cite{kingma2013auto} in 2013.
The right part of the pink component (Fig.~\ref{fig:teaser}I) was still about ``sparse,'' but ``tensor'' became a new keyword due to the increasing research interest in image data, which can be seen as a 3D tensor.
% In the red component ($\#8$), the bandit problem was still growing (Fig.~\ref{fig:text}(7)).
% Another drift also happened in the light blue component ($\#0$, Fig.~\ref{fig:teaser}J), which 
% The work ``Auto-Encoding Variational Bayes'' in 2013 
Although there were no new components, the large change of the keywords in the pink component still \yafeng{prompted} E$_3$ to adapt the model.
Since there was a noticeable drift within the pink component ($\#6$), he selected \mc{the} papers from the pink component and built a base learner with these papers.
\weikai{After the adaptation, the drift degree decreased \mc{from 0.14} to 0.08, and the performance view (Fig.~\ref{fig:teaser}F) showed that the \weikairevision{classification} accuracy increased from \textbf{0.58} to \textbf{0.74}.
Many papers about optimization (class 5) and sparse matrix (class 8) were now correctly classified.
}

\noindent\textbf{Analysis of papers in 2016-2019.}
% The last batch we added contained 3,685 papers.
As interest in machine learning increased, so did the volume of research output, leading to a large degree of drift in the model from the years 2016-2018, with the drift reaching 0.18.
After hiding \mc{some unchanged components}, the expert identified four new components.
All four new components were about deep-learning-related topics.
% To reduce visual clutter, we hide some old components with few new papers, such as \mc{which ones?}.
% to facilitate our analysis.
% The papers about DNN split and formed a new component ($\#9$) (Fig.~\ref{fig:text}(K)).
% Another new component ($\#10$) closed to it was about general deep learning techniques, with keywords of ``activation'' and ``gradient,'' (Fig.~\ref{fig:text}(K)).
%The new component ($\#11$) on the right side of the reinforcement learning component ($\#8$) was actually about deep reinforcement learning (Fig.~\ref{fig:text}(L)).
%The new component ($\#9$) on the right side of the reinforcement learning component ($\#8$) was actually about deep reinforcement learning (Fig.~\ref{fig:text}(L)).
%This new topic was triggered by the pioneering works from DeepMind on the game of Go and Atari games~\cite{mnih2015human, silver2017mastering}.
\weikai{
Component $\#9$ (Fig.~\ref{fig:text}H) was about optimization techniques for deep learning, with keywords ``gradient'' and ``sgd.''
Component $\#10$ (Fig.~\ref{fig:text}I) was about the generative adversarial network (GAN), which was first proposed in NeurIPS 2014 and quickly received much attention.
Components $\#11$ (Fig.~\ref{fig:text}J) and $\#12$ (Fig.~\ref{fig:text}K) were about recurrent neural networks (RNN) and convolutional neural networks (CNN), respectively.
These two types of deep neural networks showed great success in speech and image processing.
}
% and the component $\#13$ was mainly about ``representation'' and ``distribution'' (Fig.~\ref{fig:text}(12)).
%\weikai{To adapt to this large change of the data distribution, E$_3$ built one learner with papers in region Fig.~\ref{fig:text}K,L,M because they were all about deep models, and another learner with components $\#9$, which was about optimization.}
% the performance degradation of the model, from 0.76 to 0.64.
% Therefore, our expert needed to build some new base learners that can cover those new components.
%\mc{E$_3$ built a learner with component $\#8$ and $\#11$ because they were both about reinforcement learning, a learner with component $\#9$ and $\#10$ due to their close relation in the neural network, and other two learners with components $\#12$ and $\#13$, respectively.}
\weikai{To adapt to this large change of the data distribution, E$_3$ built a learner with the papers in the four deep-learning-related components and added it to the model.}
After the adaptation incorporating these two new learners, the \weikairevision{classification} accuracy improved from \textbf{0.59} to \textbf{0.73}, and the drift degree decreased to 0.08.

The drift degree remained nearly unchanged in 2019.
%In 2019, E3 checked the scatterplot and indeed did not found interesting new topics.
%This \yafeng{motivated} him to think about the development of machine learning in the future: is machine learning already in a bottleneck?
At the end of the case study, E3 commented that ``the trial of the system was really valuable to me not only because it solved the performance issue caused by concept drift, but also enabled me to take a wonderful tour of the past in machine learning.'' 



==> Analyzing Concept Drift in Streaming Data_2/6-discussion.tex <==
\section{Discussion and Future Work}
\label{sec:discussion}
Although the case studies on real-world datasets \yafeng{have demonstrated} the usefulness of DrifVis, there are several limitations, which may serve as promising avenues for future research.

\noindent \textbf{Generalization.}
%The generalization of DriftVis can be discussed with respect to task-wise and data-wise generalization.
In our current prototype, DriftVis has only been run on classification tasks and did not factor in known prior knowledge, if any, of the data distribution. The proposed method can be easily generalized into other tasks or to leverage known distributions, but some additional work has to be done.
%For the tasks, we currently focus on classification.
To extend to other tasks, \yafeng{such as regression or clustering,}
%such as detection, localization and regression, 
we need to replace the performance view \yafeng{with task-specific designs, e.g., RegressionExplorer~\cite{dingen2018regressionexplorer} for regression tasks}. % with a task-specific performance view.
%For example, for regression, \mc{we might want to integrate available visualization tools for regression into DriftVis, e.g., RegressionExplorer~\cite{dingen2018regressionexplorer}.} 
% we \yafeng{might want to redefine the binning approach using confidential intervals.} 
%group the data between 0 and 1 into several bins specified by the analyst.
As for the data, currently, we use an incremental GMM to model the distribution of data since it is capable of approximating any continuous distributions~\cite{bishop2006pattern}.
\yafeng{Sometimes}, the analyst \yafeng{may} have \yafeng{some} prior knowledge of the data distribution, such as using a Poisson distribution \yafeng{to better} model the accumulated event number, instead of using Gaussian distribution.
To incorporate such prior knowledge, we may consider using distribution-dependent distance functions~\cite{kifer2004detecting} in drift detection.%, such as total variation~\cite{kifer2004detecting}.
% It is desirable to improve drift detection and adaptation by combinng analysts' knowledge and the streaming data.



\noindent \textbf{Drift From Other Causes.}
In DriftVis, we focus on drift that is caused by changes in the data distribution $P(X)$, where $X$ is the data.
However, there can be concept drift due to changes in label $P(Y \mid X)$ (where $Y$ are the labels) while the data distribution $P(X)$ remains unchanged.
This is called label drift.
\mcr{For example, in the image classification task, attackers can construct adversarial examples~\cite{yuan2019adversarial} to mislead the classifier.
These adversarial examples share a similar distribution with the training data, but their label is different.}
Such drift can not be detected until the ground-truth labels are obtained.
Considering the high cost of acquiring ground-truth labels, our method focuses on the data distribution change, and label drift detection is left for future work. 
% To enable DriftVis to support label drift detection, 
To enable the support of label drift detection in DriftVis, 
two modifications are needed.
First, we can replace the distribution-based concept drift detection approach with an error-rate-based one, which relies on ground-truth labels.
Second, we can change the streaming scatterplot from visualizing $P(X)$ to showing $P(X,Y) = P(X) P(Y\mid X)$, which simultaneously covers the drift caused by $P(X)$ and  $P(Y\mid X)$.

% is the drift that the distribution $P(y\mid X)$ changes while the .

% The reason is that, in many cases, we need to stop using the models that are suffered from the concept drift before we can actually obtain the groundtruth and check its performance in new data.
% Therefore, our method is primarily developed upon distribution-based drift detection method.
% There are other drift detection method that uses error rate. 
% One promising future research could be integrating different detection techniques and taking groundtruth into effect once it is available, tho maybe partially. 
%In the future, we plan to support the detection of the actual drift once the groudtruth labels are available.

\noindent \textbf{Scalability.}
In the weather prediction case study, we demonstrated the potential of DriftVis to handle streaming data containing thousands of time points.
\weikairevision{
When there are 1,500 historical time points, the system has a latency of about 5s to process the new time point on a PC with Intel i7-9700K CPU (3.60 GHz) and 32 GB memory.}
In practice, the \mcr{incoming} data may arrive per hour, per minute, or even per second. 
%This introduces the challenge of handling streaming data with tens of thousands of time points.
As a large amount of data samples stream in rapidly, it is challenging to update the incremental GMM and the dynamic t-SNE projection fast enough for every time point, and the potentially high number of Gaussian components can make the scatterplot hard to read.
To speed up the calculation, a distribution-based sampling approach~\cite{palmer2000density} can be used. To keep the streaming scatterplot readable,
%neat and explicable,
stale or less active components can be hidden until they are activated by a certain number of new data samples.
% R2Q5
\weikairevision{Some incremental visualization techniques can also be employed to accelerate the visualization for large-scale data~\cite{fisher2012trust}.}

% \weikairevision{
% \noindent\textbf{Latency.} [I THINK IT SHOULD BE COMBINED WITH SCALABILITY AND STREAMING FUTURE WORK.]
% Take the textual data case as an example, after having processed 500 points, it takes 3 seconds to calculate the drift for all attributes and update the t-SNE layout when next 500 points come, while the time cost increase to 18 seconds after having processed 5,000 points.
% This is because we do not discard the obsolete data points in the current implementation. Therefore, the size of data that t-SNE process keeps increase and cause a large burden.
% In a streaming manner, we can discard these obsolete data points but keep their information in the aggregated form (e.g., the density map and the parameters in the GMM model) to accelerate the computation and achieve the real-time monitoring.
% }
%As the scatterplot only visualizes the data samples at recent time points, the major bottleneck lies in the efficiency of updating the incremental GMM and the scalability of the drift degree line chart.
%To handle a large number of time points, the drift degree line chart can be enhanced by archiving or stacking the oldest time points~\cite{liu2015online}.
%For the incremental GMM, a feasible approach is calculating the model parameters only from the most recent data samples and the training data.
% How should we update historical data for long time streaming data?  
% Drop stale data?

%彩蛋： no ending is our ending :( -- Yafeng
%\yafeng{With our implementation, DriftVis has made a promising step in the visualization community to assist concept drift detection, exploration, and correction. Future work would focus on developing a framework suitable for broader tasks [ROSS: BUT THIS FRAMEWORK IS PRETTY BROAD, CAN YOU GIVE SOME EXAMPLES?] and ready to incorporate expert's domain knowledge, integrating distribution-based detection and error-based detection to effectively employ any known labels and hopefully can achieve a better drift detection result, and improving system scalability for large streaming data. [MAYBE JUST END WITH SCALABILITY?] }
%\mc{Based on the above discussion, there are several interesting avenues for future research.
%First, it is promising to analyze the drift from other causes using ground-truth labels and integrated it into DriftVis.
%Another important direction is to extend DriftVis to very long streaming data containing tens of thousands of time points.
%Enabling DriftVis in incorporating analysts' prior knowledge of data distribution can also enhance user experience in different applications.}
%Thus, the third future work is to combine the knowledge-driven method with data-driven method for further improving the drift detection and adaption performance. 


% \ross{I feel like we need 3-4 sentence summary paragraph to wrap this up? Maybe not if there isn't room, just kind of ends abruptly.}

% \textbf{Categorical input?}


\section{Conclusion}

We have developed DriftVis, a visual analytics method to support the detection, examination, and correction of concept drift in streaming data. 
As part of DriftVis, we have employed an incremental GMM in the distribution-based drift detection to efficiently remove false alarms, which can be automatically addressed by the ensemble model. 
In addition to improvements in drift detection, DriftVis also introduces the streaming scatterplot visualization that uses a GMM-based constrained t-SNE and two visual modes (scatterplot and density diff) to explain different kinds of drift in the streaming data.  
DriftVis further combines drift detection, exploration, and adaptation via coordinated interactions.
%Two case studies on real-world datasets have demonstrated the usefulness of our method.
\weikairevision{A quantitative experiment and two case studies have demonstrated the usefulness of our method.}

==> Analyzing Concept Drift in Streaming Data_2/abstract.tex <==
\abstract{
Concept drift is a phenomenon in which the distribution of a data stream changes over time in unforeseen ways, causing prediction models built on historical data to become inaccurate.
While a variety of automated methods have been developed to identify when concept drift occurs, there is limited support for analysts who need to understand and correct their models when drift is detected. In this paper, we present a visual analytics method, DriftVis, to support model builders and analysts in the identification and correction of concept drift in streaming data.
DriftVis combines a distribution-based drift detection method with a streaming scatterplot to support the analysis of drift caused by the distribution changes of data streams and to explore the impact of these changes on the model's accuracy.
%precision and accuracy (ROSS: NEED HELP HERE, IS THIS PRECISION AND ACCURACY OR OTHERS).
%[NOTE: ROSS REMOVED THESE TWO SENTENCES AS THEY WERE A BIT REDUNDANT AND MAYBE GO INTO TOO MUCH DETAIL IN THE ABSTRACT, HOWEVER, IF OTHERS FEEL THEY SHOULD BE ADDED, I AM NOT OPPOSED] As streaming data is collected, DriftVis employs a drift detection method that uses a distance function to quantify the dissimilarity between the distribution of the historical data and new data to measure the drift degree.
%To help analysts identify the potential cause(s) of concept drift, a streaming scatterplot view that combines the advantages of constrained t-SNE and multi-step animation is used to support the exploration and analysis of .
%To measure the drift degree, the developed drift detection method uses a distance function to quantify the dissimilarity between the distribution of the historical data and new data.
%To explore the root cause of concept drift, the streaming scatterplot combines the advantages of the constrained t-SNE and multi-step animation.
\weikairevision{A quantitative experiment and} two case studies on weather prediction and text classification have been conducted to demonstrate our proposed tool and illustrate how visual analytics can be used to support the detection, examination, and correction of concept drift.
}

%\abstract{
%Concept drift is a phenomenon in which the distribution of a data stream changes over time in an unforeseen way, causing the prediction model built on historical data to become inaccurate.  
%To tackle this issue, we develop a visual analytics tool, DriftVis, for analyzing and understanding concept drift in %classification. 
%\shixia{streaming data}.
%DriftVis combines a distribution-based drift detection method with a streaming scatterplot to facilitate the examination of unforeseeable changes in the distribution of data streams.
%To measure the drift degree, the developed drift detection method uses a distance function to quantify the dissimilarity between the distribution of the historical data and new data.
%To explore the root cause of concept drift, the streaming scatterplot combines the advantages of the constrained t-SNE and multi-step animation.
%Two case studies are conducted to demonstrate the effectiveness and advantages of DriftVis, especially in support of the detection and understanding of concept drift.
%}

\keywords{Concept drift, streaming data, change detection, scatterplot, t-SNE.}

% One bottleneck in applying deep learning is that it is like a black box to researchers.
%deep neural networks (DNNs) have demonstrated state-of-the-art—and sometimes human-competitive results on many pattern recognition tasks, especially vision classification problems
% because progress has been hampered by the lack of understanding
% the source of their impressive performance remains poorly understood
% our understanding of how these large neural models operate has lagged behind
% Researchers most rely on anecdotal heuristics for diagnosis and refinement of deep neural networks.
%  to reduce visual clutter and extract semantic detection path of different classes
% We have applied our approach to several Twitter datasets. Qualitative evaluation and two real-world case studies demonstrate the promise of our approach for retrieving high-quality microblog data.
% The promise of our approach are demonstrated by three case studies on two benchmark datasets.
%clearly visualize connections between layers
% To reduce visual clutter we extend . for visualizing connections between layers.
% , and distribution of connections to adjacent layers as histogram
%
%

%old our method:
%We extend the current visualization of neurons to a multifaceted visualization including visualizing learned features as hierarchical rectangle packing and their activations as matrix visualization with matrix reordering.
%To reduce visual clutter we applied biclustering-based edge bundling for visualizing connections between layers.

%We applied our approach to two benchmark datasets. 

==> Analyzing Concept Drift in Streaming Data_2/conclusion.tex <==
% !TEX root = EvoTree-KDD.tex

\section{Conclusion}\label{sec:conclustion}
\label{sec:conclusion}


==> conclusion.tex <==
% !TEX root = EvoTree-KDD.tex

\section{Conclusion}\label{sec:conclustion}
\label{sec:conclusion}

